Grade Like a Human: Rethinking Automated Assessment with Large Language Models

While large language models (LLMs) have been used for automated grading, they have not yet achieved the same level of performance as humans, especially when it comes to grading complex questions. Existing research on this topic focuses on a particular step in the grading procedure: grading using predefined rubrics. However, grading is a multifaceted procedure that encompasses other crucial steps, such as grading rubrics design and post-grading review. There has been a lack of systematic research exploring the potential of LLMs to enhance the entire grading~process. In this paper, we propose an LLM-based grading system that addresses the entire grading procedure, including the following key components: 1) Developing grading rubrics that not only consider the questions but also the student answers, which can more accurately reflect students' performance. 2) Under the guidance of grading rubrics, providing accurate and consistent scores for each student, along with customized feedback. 3) Conducting post-grading review to better ensure accuracy and fairness. Additionally, we collected a new dataset named OS from a university operating system course and conducted extensive experiments on both our new dataset and the widely used Mohler dataset. Experiments demonstrate the effectiveness of our proposed approach, providing some new insights for developing automated grading systems based on LLMs.

==> Styles/table.tex <==
\section{Experiments}
\label{s:exp}

In this section, we implement our system and test it using the \ourdataset~dataset mentioned in Section \ref{s:os_dataset}, as well as an open-source dataset, Mohler~\citep{mohler2011learning,mohler2009text}. 
The Mohler dataset is a question-answer grading database in the ASAG field, with questions pertaining to computer science. The organization of the Mohlar dataset is identical to the \ourdataset~dataset shown in Figure \ref{fig:example_os}, but it does not include grading criteria. A more detailed introduction can be found in Appendix~\ref{appendix:mohler}.
Our system is deployed on a server equipped with two A100 GPUs and 400GB of memory.
When implementing our system, we utilized OpenAI's API~\cite{openai-api} as our LLM source, and employed LangChain~\cite{langchain} to implement the agents and workflows. 
To objectively evaluate our system's performance in the grading task, we used multiple evaluation metrics, including MAE and RMSE, among others. These metrics are detailed in Appendix~\ref{Appendix:eval_metric}. 
\xwj{Add exlain for "bar error" like:"In this paper, all experimental results represent the average of multiple repeated experiments.
}


\subsection{Evaluations of Various Generated Rubrics}


We first evaluate the impact of different rubrics on the grading effectiveness of LLMs and simultaneously verify the effectiveness of the algorithm proposed in Section~\ref{s-gencri}.
Table~\ref{tab-gencri} presents the evaluation results on the \ourdataset~dataset, while Table~\ref{tab-gencri-mohler} shows the evaluation results on the Mohler dataset.


The evaluation on the \ourdataset~dataset includes four different grading rubrics. Among them, the \textbf{Coarse-gr., TA} and \textbf{Fine-gr., TA} rubrics are both manually generated rubrics that we followed when scoring student answers. 
The difference is the granularity: The former provides only the standard answer, while the latter additionally includes a grading criteria, as illustrated in Figure~\ref{fig:example_os}. \textbf{Gen., Rand.} and \textbf{Gen., Distr.} are respectively derived from the two rubric generation algorithms we demonstrated in Section~\ref{s-gencri}.
The rubrics for the Mohler dataset differ. Since the Mohler dataset does not provide grading criteria, it includes only two rubrics: \textbf{Coarse-gr.}, which directly comes from the standard answer for each question included in the dataset, and \textbf{Fine-gr.}, which is generated using the rubric generation algorithm.
In Appendix~\ref{appendix:rubric}, we present several examples to illustrate the different rubrics.


% \paragraph{Rubric Granularity v.s. Performance}
We compared the performance using different granularities of rubrics. In Tables~\ref{tab-gencri} and~\ref{tab-gencri-mohler}, we observed completely opposite phenomena: for the \ourdataset~dataset, fine-grained rubrics significantly improved scoring performance, whereas for the Mohler dataset, fine-grained rubrics actually reduced scoring performance.
%
We attribute it to the differing difficulties of the two datasets. 
For the OS dataset, each question is relatively long and complex, involving multiple steps and often including code execution. For such problems, LLMs lack sufficient capability to provide correct answers on their own, so detailed rubrics help LLMs score correctly.
In contrast, the questions in the Mohler dataset are relatively simple. For example, one question in the Mohler dataset is: \textit{``What is the role of a prototype program in problem solving?''}
For such questions, the world knowledge of LLMs is sufficient to provide good answers, as well as to evaluate students' responses. Therefore, not overly constraining the LLMs can better leverage their abilities~\cite{patil2023gorilla}.
% 
Additionally, in Table~\ref{tab-gencri}, we further observe that our rubric generation algorithm can further improve the grading performance on complex questions.
%
Based on this, we claim that our approach is effective for complex problems and further demonstrate the importance of our \ourdataset~dataset for better evaluating the performance of LLMs on grading tasks.
%
Therefore, in the subsequent evaluation, we mainly focus on the improvements our method brings to the \ourdataset~dataset.

% In Table~\ref{tab-gencri}, we compare the performance of \textbf{Fine-gr., TA} and \textbf{Coarse-gr., TA}. The results show that the scores achieved with the \textbf{Fine-gr., TA} are better, indicating that, on the OS dataset, providing more detailed grading criteria can help LLMs learn the human-expected grading rules more effectively.
% When comparing the rubrics generated using our proposed sampling methods (\textbf{Gen., Rand.} and \textbf{Gen., Distr.}) with those specified by TAs (\textbf{Coarse-gr., TA} and \textbf{Fine-gr., TA}) at different granularities, our method-produced rubrics demonstrate superior grading performance. This validates the effectiveness of our iterative rubric generation based on actual student responses in improving rubric quality. Additionally, the \textbf{Gen., Distr.} rubric achieves the best grading performance across all questions.

% Moreover, in the Mohler dataset, as shown in~\ref{tab-gencri-mohler}, the \textbf{Fine-gr.} rubric yields worse grading performance compared to the \textbf{Coarse-gr.} rubric. This result suggests that overly detailed grading rubrics can sometimes misguide the LLMs, especially when grading simple questions and short student responses, leading to more errors. This further supports the necessity of iteratively optimizing the rubric in our grading framework, based on the specific questions and actual student responses.


%  In this paper, we evaluate the impact of different grading rubrics on grading results using the OS dataset we collected, as shown in Table \ref{tab-gencri}.
%  Table \ref{tab-gencri-mohler} presents the grading results of different types of grading rubrics on the Mohler dataset.


% The first two type rubrics in the table represent rubrics formulated by the expert teachers (TA) of the OS course. The \emph{Coarse-grained} rubric provides a relatively broad grading scale, indicating the number of sub-questions and their corresponding scores.
% The \emph{Fine-grained} rubric adds specific grading criteria and rules for each sub-question, building upon the Coarse-grained rubric. The \emph{Random} and \emph{Distribution} type rubrics correspond to the two methods for generating rubrics by LLMs discussed in Section ~\ref{s-gencri}. (Examples of various types of rubric content can be found in the Appendix ~\ref{appendix:rubric})

% We can observe the following from table ~\ref{tab-gencri}:

% \begin{enumerate}
%     \item Compared to the Coarse-grained rubric, the Fine-grained rubric exhibits smaller scoring errors on LLMs and demonstrates a stronger correlation with human grading. This suggests that a more detailed grading rubric leads to better grading accuracy performance on LLMs.
%     \item Compared to the rubric formulated by the expert teachers, the grading rubrics generated using the proposed Random and Distribution methods significantly improve the quality of grading, with the Distribution method showing greater enhancement. This validates the effectiveness of the proposed strategy in combining LLMs with real student responses to generate grading rubrics.
% \end{enumerate}

%  We can observe that setting a more detailed grading rubric actually leads to a significant decrease in grading accuracy performance. This finding aligns with our earlier point, demonstrating that for particularly simple questions and short student responses, a detailed grading rubric can restrict the ability of LLMs during the grading process. 


%  Due to the relatively simple nature of the questions in the Mohler dataset, which mainly assess concepts in computer science, the student responses are typically shorter in length. As a result, it is not suitable to use overly complex grading rubrics. 
 
% When utilizing LLMs for grading tasks, different types of data may require different types of grading rubric. It is important to flexibly adjust the rubric based on the specific circumstances in order to choose the most suitable rubric.



\begin{table}[htbp]
\centering
\caption{Results obtained on OS dataset}
\label{tab-gencri}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
 & \multicolumn{4}{c}{\textit{Q1}} &  & \multicolumn{4}{c}{\textit{Q2}} \\ \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 6.97 & 8.98 & 0.47 & 0.46 &  & 5.90 & 7.57 & 0.47 & 0.10 \\
\textbf{Fine-gr., TA} &  4.51 & 5.62 & 0.30 & 0.74 &  & 5.90 & 7.75 & 0.48 & 0.15 \\
\textbf{Gen., Rand.} & 4.42 & 5.65 & 0.30 & 0.75 &  & 5.95 & 7.65 & 0.48 & 0.32 \\
\textbf{Gen., Distr.} & \textbf{4.05} & \textbf{5.21} & \textbf{0.27} & \textbf{0.76} &  & \textbf{5.70}  & \textbf{7.46}  & \textbf{0.47} & \textbf{0.37} \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q3}} &  & \multicolumn{4}{c}{\textit{Q4}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 2.85 & 3.41 & 0.23 & 0.62 &  & 5.45 & 7.32 & 0.46 & 0.36 \\
\textbf{Fine-gr., TA} & 2.40 & 3.38 & 0.23 & 0.71 &  & 4.78 & 6.25 & 0.39 & 0.45 \\
\textbf{Gen., Rand.} & 2.50 & 3.50 & 0.23 & 0.72 &  & 4.10 & 5.83 & 0.36 & 0.55 \\
\textbf{Gen., Distr.} & \textbf{2.35} & \textbf{3.17} & \textbf{0.21} & \textbf{0.75} &  & \textbf{3.38} & \textbf{4.89}  & \textbf{0.31} & \textbf{0.60} \\ % \hline  % \hline
 & \multicolumn{4}{c}{\textit{Q5}} &  & \multicolumn{4}{c}{\textit{Q6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 10.90 & 13.10 & 0.49 & 0.53 &  & 9.22 & 12.86 & 0.32 & 0.42 \\
\textbf{Fine-gr., TA} & 9.62 & 11.77 & 0.44 & 0.49 &  & 10.55 & 12.83 & 0.32 & 0.47 \\
\textbf{Gen., Rand.} & 6.05 & 8.41 & 0.31 & 0.64 &  & 9.62 & 12.62 & 0.32 & 0.40 \\
\textbf{Gen., Distr.} & \textbf{6.03} & \textbf{8.21} & \textbf{0.30}  & \textbf{0.66} &  & \textbf{8.72} & \textbf{11.42} & \textbf{0.29} & \textbf{0.50} \\ \hline
\end{tabular}%
}
\end{table}
%%
\begin{table}[htbp]
\centering
\caption{Results obtained on Mohler dataset}
\label{tab-gencri-mohler}
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline  \hline
 & \multicolumn{4}{c}{\textit{Q1.1}} &  & \multicolumn{4}{c}{\textit{Q2.6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.78} & \textbf{1.02} & \textbf{0.29} & \textbf{0.69} & & \textbf{0.90} & \textbf{1.11} & \textbf{0.37} & \textbf{0.34}   \\
\textbf{Fine-gr.} & 1.67  & 2.06 & 0.59 & 0.03 & & 1.83 &  2.00 & 0.67 & 0.37 \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q2.7}} &  & \multicolumn{4}{c}{\textit{Q3.6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.59} & \textbf{0.74} & \textbf{0.15} & \textbf{0.15} &  & \textbf{0.43} & \textbf{0.87} & \textbf{0.35} & \textbf{0.60} \\
\textbf{Fine-gr.} & 0.90 & 1.11 & 0.22 & 0.55 &  & 0.61 & 1.21 & 0.45 & 0.53 \\%  \hline % \hline
 & \multicolumn{4}{c}{\textit{Q4.2}} &  & \multicolumn{4}{c}{\textit{Q11.7}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.57} & \textbf{0.80} & \textbf{0.27} & \textbf{0.68} &  & \textbf{0.68} & \textbf{0.80} & \textbf{0.28} & \textbf{0.74} \\
\textbf{Fine-gr.} & 0.50 & 0.89 & 0.30 & 0.64 &  & 0.72 & 0.97 & 0.31 & 0.68 \\ \hline
\end{tabular}%
}
\end{table}
%%
\begin{table}[]
\centering
\caption{Results of different prompts on OS dataset}
\label{tab-prompts}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
 & \multicolumn{4}{c}{\textit{Q1, batch size=10}} &  & \multicolumn{4}{c}{\textit{Q2, batch size=40}} \\ \cline{2-5} \cline{7-10} 
\textbf{Baseline} & 4.28 & 5.81 & 0.31 & 0.73 &  & 7.35 & 9.58 & 0.60 & 0.30 \\
\textbf{One-shot} &  3.74 & 5.33& 0.28 & 0.77 &  & 5.70 & 7.46 & 0.47 & 0.37 \\
\textbf{Self-reflection} & 3.83 & 4.98 & 0.26 & 0.76 &  & 5.95 & 7.68 & 0.48 & 0.36 \\
\textbf{Batching} & \textbf{3.59} & \textbf{4.64} & \textbf{0.24} & \textbf{0.79} & & \textbf{3.09} & \textbf{6.28} & \textbf{0.39} & \textbf{0.42} \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q3, batch size=40}} &  & \multicolumn{4}{c}{\textit{Q4, batch size=30}} \\  \cline{2-5} \cline{7-10} 
\textbf{Baseline} & 2.00 & 2.89 & 0.19 & 0.74 &  & 3.33 & 5.48 & 0.34 & 0.46 \\
\textbf{One-shot} &  \textbf{1.95} & \textbf{2.72} & \textbf{0.18} & \textbf{0.79} &  & \textbf{3.23} & \textbf{4.81} & \textbf{0.30} & \textbf{0.59} \\
\textbf{Self-reflection} &  2.55 &  3.21 & 0.21 & 0.74 &  & 3.85 & 5.55 &  0.35 &0.42 \\
\textbf{Batching} & 2.98 & 3.95 & 0.26 & 0.44 & & 3.83 & 5.93 & 0.37 & 0.32 \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q5, batch size=40}} &  & \multicolumn{4}{c}{\textit{Q6, batch size=20}} \\  \cline{2-5} \cline{7-10} 
 \textbf{Baseline} & 6.00 & 8.07 & 0.30 & 0.66 &  & 11.00 & 14.6 & 0.36 & \textbf{0.22} \\
\textbf{One-shot} &  \textbf{4.15} & \textbf{6.07} & \textbf{0.22} & \textbf{0.78} &  & \textbf{7.95} & \textbf{10.23} & \textbf{0.26} & \textbf{0.22} \\
\textbf{Self-reflection} & 7.33 & 9.46 & 0.35 & 0.57 &  & 10.90 & 14.53 & 0.36 & \textbf{0.22} \\
\textbf{Batching} & 8.20 & 10.33 & 0.38 & 0.63 & & 11.91 & 16.45 & 0.41 & 0.21 \\ \hline 
\end{tabular}%
}
\end{table}
%%



\subsection{Evaluations of Prompt Strategies in Grading}
\label{s:eval_prompts}


In this section, we assess the impact of different prompting strategies on performance during the grading process. The evaluation results are presented in Table~\ref{tab-prompts} (\emph{batch size} corresponds to the setting of the Batching prompts).
%
For all questions in the \ourdataset~dataset, our prompting strategies exceeded the baseline levels. 
The results indicate that different questions have different optimal prompting strategies, with Batching and One-Shot performing the best among all strategies. We also observed that, in certain cases, some strategies could reduce the grading performance. These observations suggest that it is crucial to design different prompting strategies tailored to the characteristics of specific questions.



% The results in Table~\ref{tab-selfreflection} shows the performance of the self-reflection prompt on the OS dataset. Notably, we observe variations in grading accuracy across different questions. Specifically, for questions \textit{Q1}, \textit{Q2} and \textit{Q6}, the self-reflection prompt achieves better grading accuracy compared to the baseline's initial performance.
% However, for questions \textit{Q3}, \textit{Q4} and \textit{Q5}, the grading results following self-reflection are worse than the baseline's initial performance. This variability underscores the question-dependent nature of LLMs' self-reflection ability in grading tasks.
% These findings highlight the importance of analyzing each question individually in the grading process. It emphasizes the inadequacy of employing a universal prompt strategy to achieve consistently high grading results across all question types. Instead, a flexible approach is warranted, wherein different strategies are adopted based on the specific characteristics of each problem.

% Moreover, these results validate the necessity of our proposed systematic and multi-agent grading framework, which allows for adaptable and context-specific grading strategies tailored to the nuances of each question.


% \xwj{Batching Table , add a note to explain the batch size value setting, like : Due to the token length limitation and varying lengths of questions and student answers for each question, the maximum batch size for grading differs for each question within the allowable token length range.}

% Table \ref{tab-batchos} and Table \ref{tab-batchmohler} show the grading results of the batching strategy on the OS dataset and the Mohler dataset, respectively. On the OS dataset, we find that the impact of the batching strategy on the grading performance across different questions is similar to the impact of the self-reflection strategy (as shown in Table \ref{tab-selfreflection}). Specifically, for $q_1$, $q_2$, $q_4$, and $q_5$, the grading accuracy with batching is better than without batching. However, for $q_3$ and $q_6$, the grading results with batching are better.
% On the Mohler dataset, we observe that the performance of the without batching prompt is better than the with batching approach.
% These findings further reinforce the point we claim based on the results in Table \ref{tab-selfreflection}, indicating that the effectiveness of some prompt strategies, such as self-reflection and batching, is highly dependent on the specific characteristics of the assessment tasks.
% The grading results from Table~\ref{tab-batchos} for the OS dataset and Table~\ref{tab-batchmohler} for the Mohler dataset shed light on our batching strategy's impact. 
% We find that effects of the batching strategy on the OS dataset closely resemble those observed with the self-reflection strategy as detailed in Table~\ref{tab-selfreflection}. Specifically, for questions \textit{Q1}, \textit{Q2}, \textit{Q4}, and \textit{Q5}, grading accuracy improves with batching compared to without batching. Conversely, for \textit{Q3} and \textit{Q6}, grading results without batching are better. 
% On the Mohler dataset, grading results without batching outperform those with batching, corroborating our point from Table~\ref{tab-selfreflection}. This highlights that the efficacy of prompt strategies like self-reflection and batching depends on assessment task characteristics.



\subsection{Evaluations for Score Review}



\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \caption{Evaluation of re-grouping strategy}
    \label{tab-regroup}
    \resizebox{.55\textwidth}{!}{%
        \begin{tabular}{rcccccc}
        \hline
         & \multicolumn{6}{c}{\textbf{Accuracy $\uparrow$}} \\ \cline{2-7} 
        \textbf{Methods} & \textit{Q1} & \textit{Q2} & \textit{Q3} & \textit{Q4} & \textit{Q5} & \textit{Q6} \\ \hline
        \textbf{Baseline} & 0.58 & 0.64 & 0.59 & 0.72 & 0.55 & 0.70 \\
        \textbf{Re-grouping} & \textbf{0.62} & \textbf{0.73} & \textbf{0.71} & \textbf{0.77} & \textbf{0.64} & \textbf{0.76} \\ \hline
        \end{tabular}
    }
\end{wraptable}

In this section, we evaluate the impact of the review process on grading performance and the effectiveness of re-grouping strategies in improving the accuracy of identifying unreasonable results. 
%
During the testing process, we randomly selected some students and modified their scores to simulate the occurrence of unreasonable results. The evaluation results are presented in Table~\ref{tab-regroup}.
%
The results show that through the review process, the LLM can detect anomalies in the grading, thereby further improving the accuracy. Additionally, the re-grouping strategy can further enhance the model's accuracy.


% For the OS dataset, which was manually annotated, each question comprises a total of 40 student responses, with the average of three grades serving as the correct ground truth label for each response.
% To simulate instances of erroneous scoring, we randomly selected 5 student responses for each question and constructed anomalous scores for these samples. This process allowed us to create a dataset containing instances of scoring errors.
% Subsequently, we employed the method proposed in Section~\ref{s:score_review} to leverage the GPT-3.5 model in identifying cases of anomalous scoring. By doing so, we aimed to evaluate the model's capacity to detect instances where the assigned score deviated from the correct ground truth label. This evaluation is crucial within the context of score review and quality assurance, as it enables us to assess the model's effectiveness in identifying scoring discrepancies.


\iffalse
这部分实验数据支撑比较少，我倾向于弱化实验效果， 强调提供一种新的思路：对input data的组织方式也会影响LLMs的任务效果。
\fi
% The experiment implementation details of this part can be found in the Appendix \ref{appedix:score_review}. Table \ref{tab-regroup} shows the performance of the regroup strategy on the score review task. Compared to the baseline method, our proposed regroup strategy achieved better accuracy performance in identifying anomalous scoring cases.
% Our main goal is to provide a new idea to constructing prompt strategies: The way we organize the input data can also influence the performance of LLMs on specific tasks, such as the score review task.
% In the future, we will continue to conduct related work to further explore this issue in depth. 









While large language models (LLMs) have been used for automated grading, they have not yet achieved the same level of performance as humans, especially when it comes to grading complex questions. 
Existing research on this topic focuses on a particular step in the grading procedure: grading using predefined rubrics. However, grading is a multifaceted procedure that encompasses other crucial steps, such as grading rubrics design and post-grading review. There has been a lack of systematic research exploring the potential of LLMs to enhance the entire grading~process.

In this paper, we propose an LLM-based grading system that addresses the entire grading procedure, including the following key components:
1) Developing grading rubrics that not only consider the questions but also the student answers, which can more accurately reflect students' performance.
2) Under the guidance of grading rubrics, providing accurate and consistent scores for each student, along with customized feedback.
3) Conducting post-grading review to better ensure accuracy and fairness.
Additionally, we collected a new dataset named \ourdataset~from a university operating system course and conducted extensive experiments on both our new dataset and the widely used Mohler dataset. Experiments demonstrate the effectiveness of our proposed approach, providing some new insights for developing automated grading systems based on LLMs.


==> exp.tex <==
\section{Experiments}
\label{s:exp}

In this section, we implement our system and test it using the \ourdataset~dataset mentioned in Section \ref{s:os_dataset}, as well as an open-source dataset, Mohler~\citep{mohler2011learning,mohler2009text}. 
The Mohler dataset is a question-answer grading database in the ASAG field, with questions pertaining to computer science. The organization of the Mohlar dataset is identical to the \ourdataset~dataset shown in Figure \ref{fig:example_os}, but it does not include grading criteria. A more detailed introduction can be found in Appendix~\ref{appendix:mohler}.
Our system is deployed on a server equipped with two A100 GPUs and 400GB of memory.
When implementing our system, we utilized OpenAI's API~\cite{openai-api} as our LLM source, and employed LangChain~\cite{langchain} to implement the agents and workflows. 
To objectively evaluate our system's performance in the grading task, we used multiple evaluation metrics, including MAE and RMSE, among others. These metrics are detailed in Appendix~\ref{Appendix:eval_metric}. 
Since the outputs of LLMs inherently possess uncertainty, during experiments, each metric is measured multiple times and the average value is presented as the result.


\subsection{Evaluations of Various Generated Rubrics}





%%%table 1
\begin{table}[]
\centering
\caption{The grading performance under different rubric generation methods for the \ourdataset~dataset}
\label{tab-gencri}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
 & \multicolumn{4}{c}{\textit{Q1}} &  & \multicolumn{4}{c}{\textit{Q2}} \\ \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 6.97 & 8.98 & 0.47 & 0.46 &  & 5.90 & 7.57 & \textbf{0.47} & 0.10 \\
\textbf{Fine-gr., TA} &  4.51 & 5.62 & 0.30 & 0.74 &  & 5.90 & 7.75 & 0.48 & 0.15 \\
\textbf{Gen., Rand.} & 4.42 & 5.65 & 0.30 & 0.75 &  & 5.95 & 7.65 & 0.48 & 0.32 \\
\textbf{Gen., Distr.} & \textbf{4.05} & \textbf{5.21} & \textbf{0.27} & \textbf{0.76} &  & \textbf{5.70}  & \textbf{7.46}  & \textbf{0.47} & \textbf{0.37} \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q3}} &  & \multicolumn{4}{c}{\textit{Q4}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 2.85 & 3.41 & 0.23 & 0.62 &  & 5.45 & 7.32 & 0.46 & 0.36 \\
\textbf{Fine-gr., TA} & 2.40 & 3.38 & 0.23 & 0.71 &  & 4.78 & 6.25 & 0.39 & 0.45 \\
\textbf{Gen., Rand.} & 2.50 & 3.50 & 0.23 & 0.72 &  & 4.10 & 5.83 & 0.36 & 0.55 \\
\textbf{Gen., Distr.} & \textbf{2.35} & \textbf{3.17} & \textbf{0.21} & \textbf{0.75} &  & \textbf{3.38} & \textbf{4.89}  & \textbf{0.31} & \textbf{0.60} \\ % \hline  % \hline
 & \multicolumn{4}{c}{\textit{Q5}} &  & \multicolumn{4}{c}{\textit{Q6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 10.90 & 13.10 & 0.49 & 0.53 &  & 9.22 & 12.86 & 0.32 & 0.42 \\
\textbf{Fine-gr., TA} & 9.62 & 11.77 & 0.44 & 0.49 &  & 10.55 & 12.83 & 0.32 & 0.47 \\
\textbf{Gen., Rand.} & 6.05 & 8.41 & 0.31 & 0.64 &  & 9.62 & 12.62 & 0.32 & 0.40 \\
\textbf{Gen., Distr.} & \textbf{6.03} & \textbf{8.21} & \textbf{0.30}  & \textbf{0.66} &  & \textbf{8.72} & \textbf{11.42} & \textbf{0.29} & \textbf{0.50} \\ \hline
\end{tabular}%
}
\end{table}
%% table 2
\begin{table}[]
\centering
\caption{The grading performance under different rubric generation methods for the Mohler dataset}
\label{tab-gencri-mohler}
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline  \hline
 & \multicolumn{4}{c}{\textit{Q1.1}} &  & \multicolumn{4}{c}{\textit{Q2.6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.78} & \textbf{1.02} & \textbf{0.29} & \textbf{0.69} & & \textbf{0.90} & \textbf{1.11} & \textbf{0.37} & \textbf{0.34}   \\
\textbf{Fine-gr.} & 1.67  & 2.06 & 0.59 & 0.03 & & 1.83 &  2.00 & 0.67 & 0.37 \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q2.7}} &  & \multicolumn{4}{c}{\textit{Q3.6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.59} & \textbf{0.74} & \textbf{0.15} & \textbf{0.65} &  & \textbf{0.43} & \textbf{0.87} & \textbf{0.35} & \textbf{0.60} \\
\textbf{Fine-gr.} & 0.90 & 1.11 & 0.22 & 0.55 &  & 0.61 & 1.21 & 0.45 & 0.53 \\%  \hline % \hline
 & \multicolumn{4}{c}{\textit{Q4.2}} &  & \multicolumn{4}{c}{\textit{Q11.7}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.57} & \textbf{0.80} & \textbf{0.27} & \textbf{0.68} &  & \textbf{0.68} & \textbf{0.80} & \textbf{0.28} & \textbf{0.74} \\
\textbf{Fine-gr.} & 0.50 & 0.89 & 0.30 & 0.64 &  & 0.72 & 0.97 & 0.31 & 0.68 \\ \hline
\end{tabular}%
}
\end{table}

We first evaluate the impact of different rubrics on the grading effectiveness of LLMs and simultaneously verify the effectiveness of the algorithm proposed in Section~\ref{s-gencri}.
Table~\ref{tab-gencri} presents the evaluation results on the \ourdataset~dataset, while Table~\ref{tab-gencri-mohler} shows the evaluation results on the Mohler dataset.


The evaluation on the \ourdataset~dataset includes four different grading rubrics. Among them, the \textbf{Coarse-gr., TA} and \textbf{Fine-gr., TA} rubrics are both manually generated rubrics that we followed when scoring student answers. 
The difference is the granularity: The former provides only the standard answer, while the latter additionally includes a grading criteria, as illustrated in Figure~\ref{fig:example_os}. \textbf{Gen., Rand.} and \textbf{Gen., Distr.} are respectively derived from the two rubric generation algorithms we demonstrated in Section~\ref{s-gencri}.
The rubrics for the Mohler dataset differ. Since the Mohler dataset does not provide grading criteria, it includes only two rubrics: \textbf{Coarse-gr.}, which directly comes from the standard answer for each question included in the dataset, and \textbf{Fine-gr.}, which is generated using the rubric generation algorithm.
In Appendix~\ref{appendix:rubric}, we present several examples to illustrate the different rubrics.


% \paragraph{Rubric Granularity v.s. Performance}
We compared the performance using different granularities of rubrics. In Tables~\ref{tab-gencri} and~\ref{tab-gencri-mohler}, we observed completely opposite phenomena: for the \ourdataset~dataset, fine-grained rubrics significantly improved scoring performance, whereas for the Mohler dataset, fine-grained rubrics actually reduced scoring performance.
%
We attribute it to the differing difficulties of the two datasets. 
For the OS dataset, each question is relatively long and complex, involving multiple steps and often including code execution. For such problems, LLMs lack sufficient capability to provide correct answers on their own, so detailed rubrics help LLMs score correctly.
In contrast, the questions in the Mohler dataset are relatively simple. For example, one question in the Mohler dataset is: \textit{``What is the role of a prototype program in problem solving?''}
For such questions, the world knowledge of LLMs is sufficient to provide good answers, as well as to evaluate students' responses. Therefore, not overly constraining the LLMs can better leverage their abilities~\cite{patil2023gorilla}.
% 
Additionally, in Table~\ref{tab-gencri}, we further observe that our rubric generation algorithm can further improve the grading performance on complex questions.
%
Based on this, we claim that our approach is effective for complex problems and further demonstrate the importance of our \ourdataset~dataset for better evaluating the performance of LLMs on grading tasks.
%
Therefore, in the subsequent evaluation, we mainly focus on the improvements our method brings to the \ourdataset~dataset.

% In Table~\ref{tab-gencri}, we compare the performance of \textbf{Fine-gr., TA} and \textbf{Coarse-gr., TA}. The results show that the scores achieved with the \textbf{Fine-gr., TA} are better, indicating that, on the OS dataset, providing more detailed grading criteria can help LLMs learn the human-expected grading rules more effectively.
% When comparing the rubrics generated using our proposed sampling methods (\textbf{Gen., Rand.} and \textbf{Gen., Distr.}) with those specified by TAs (\textbf{Coarse-gr., TA} and \textbf{Fine-gr., TA}) at different granularities, our method-produced rubrics demonstrate superior grading performance. This validates the effectiveness of our iterative rubric generation based on actual student responses in improving rubric quality. Additionally, the \textbf{Gen., Distr.} rubric achieves the best grading performance across all questions.

% Moreover, in the Mohler dataset, as shown in~\ref{tab-gencri-mohler}, the \textbf{Fine-gr.} rubric yields worse grading performance compared to the \textbf{Coarse-gr.} rubric. This result suggests that overly detailed grading rubrics can sometimes misguide the LLMs, especially when grading simple questions and short student responses, leading to more errors. This further supports the necessity of iteratively optimizing the rubric in our grading framework, based on the specific questions and actual student responses.


%  In this paper, we evaluate the impact of different grading rubrics on grading results using the OS dataset we collected, as shown in Table \ref{tab-gencri}.
%  Table \ref{tab-gencri-mohler} presents the grading results of different types of grading rubrics on the Mohler dataset.


% The first two type rubrics in the table represent rubrics formulated by the expert teachers (TA) of the OS course. The \emph{Coarse-grained} rubric provides a relatively broad grading scale, indicating the number of sub-questions and their corresponding scores.
% The \emph{Fine-grained} rubric adds specific grading criteria and rules for each sub-question, building upon the Coarse-grained rubric. The \emph{Random} and \emph{Distribution} type rubrics correspond to the two methods for generating rubrics by LLMs discussed in Section ~\ref{s-gencri}. (Examples of various types of rubric content can be found in the Appendix ~\ref{appendix:rubric})

% We can observe the following from table ~\ref{tab-gencri}:

% \begin{enumerate}
%     \item Compared to the Coarse-grained rubric, the Fine-grained rubric exhibits smaller scoring errors on LLMs and demonstrates a stronger correlation with human grading. This suggests that a more detailed grading rubric leads to better grading accuracy performance on LLMs.
%     \item Compared to the rubric formulated by the expert teachers, the grading rubrics generated using the proposed Random and Distribution methods significantly improve the quality of grading, with the Distribution method showing greater enhancement. This validates the effectiveness of the proposed strategy in combining LLMs with real student responses to generate grading rubrics.
% \end{enumerate}

%  We can observe that setting a more detailed grading rubric actually leads to a significant decrease in grading accuracy performance. This finding aligns with our earlier point, demonstrating that for particularly simple questions and short student responses, a detailed grading rubric can restrict the ability of LLMs during the grading process. 


%  Due to the relatively simple nature of the questions in the Mohler dataset, which mainly assess concepts in computer science, the student responses are typically shorter in length. As a result, it is not suitable to use overly complex grading rubrics. 
 
% When utilizing LLMs for grading tasks, different types of data may require different types of grading rubric. It is important to flexibly adjust the rubric based on the specific circumstances in order to choose the most suitable rubric.



% \begin{table}[htbp]
% \centering
% \caption{Results obtained on OS dataset}
% \label{tab-gencri}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rccccccccc}
% \hline
% \rule{0pt}{1.1em} % 设置行高
%  \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
%  & \multicolumn{4}{c}{\textit{Q1}} &  & \multicolumn{4}{c}{\textit{Q2}} \\ \cline{2-5} \cline{7-10} 
% \textbf{Coarse-gr., TA} & 6.97 & 8.98 & 0.47 & 0.46 &  & 5.90 & 7.57 & 0.47 & 0.10 \\
% \textbf{Fine-gr., TA} &  4.51 & 5.62 & 0.30 & 0.74 &  & 5.90 & 7.75 & 0.48 & 0.15 \\
% \textbf{Gen., Rand.} & 4.42 & 5.65 & 0.30 & 0.75 &  & 5.95 & 7.65 & 0.48 & 0.32 \\
% \textbf{Gen., Distr.} & \textbf{4.05} & \textbf{5.21} & \textbf{0.27} & \textbf{0.76} &  & \textbf{5.70}  & \textbf{7.46}  & \textbf{0.47} & \textbf{0.37} \\ % \hline % \hline
%  & \multicolumn{4}{c}{\textit{Q3}} &  & \multicolumn{4}{c}{\textit{Q4}} \\  \cline{2-5} \cline{7-10} 
% \textbf{Coarse-gr., TA} & 2.85 & 3.41 & 0.23 & 0.62 &  & 5.45 & 7.32 & 0.46 & 0.36 \\
% \textbf{Fine-gr., TA} & 2.40 & 3.38 & 0.23 & 0.71 &  & 4.78 & 6.25 & 0.39 & 0.45 \\
% \textbf{Gen., Rand.} & 2.50 & 3.50 & 0.23 & 0.72 &  & 4.10 & 5.83 & 0.36 & 0.55 \\
% \textbf{Gen., Distr.} & \textbf{2.35} & \textbf{3.17} & \textbf{0.21} & \textbf{0.75} &  & \textbf{3.38} & \textbf{4.89}  & \textbf{0.31} & \textbf{0.60} \\ % \hline  % \hline
%  & \multicolumn{4}{c}{\textit{Q5}} &  & \multicolumn{4}{c}{\textit{Q6}} \\  \cline{2-5} \cline{7-10} 
% \textbf{Coarse-gr., TA} & 10.90 & 13.10 & 0.49 & 0.53 &  & 9.22 & 12.86 & 0.32 & 0.42 \\
% \textbf{Fine-gr., TA} & 9.62 & 11.77 & 0.44 & 0.49 &  & 10.55 & 12.83 & 0.32 & 0.47 \\
% \textbf{Gen., Rand.} & 6.05 & 8.41 & 0.31 & 0.64 &  & 9.62 & 12.62 & 0.32 & 0.40 \\
% \textbf{Gen., Distr.} & \textbf{6.03} & \textbf{8.21} & \textbf{0.30}  & \textbf{0.66} &  & \textbf{8.72} & \textbf{11.42} & \textbf{0.29} & \textbf{0.50} \\ \hline
% \end{tabular}%
% }
% \end{table}

%% table 3
\begin{table}[t]
\centering
\caption{The impact of different prompt strategies on grading performance for the \ourdataset~dataset}
\label{tab-prompts}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
 & \multicolumn{4}{c}{\textit{Q1, batch size=10}} &  & \multicolumn{4}{c}{\textit{Q2, batch size=40}} \\ \cline{2-5} \cline{7-10} 
\textbf{Baseline} & 4.28 & 5.81 & 0.31 & 0.73 &  & 7.35 & 9.58 & 0.60 & 0.30 \\
\textbf{One-shot} &  3.74 & 5.33& 0.28 & 0.77 &  & 5.70 & 7.46 & 0.47 & 0.37 \\
\textbf{Self-reflection} & 3.83 & 4.98 & 0.26 & 0.76 &  & 5.95 & 7.68 & 0.48 & 0.36 \\
\textbf{Batching} & \textbf{3.59} & \textbf{4.64} & \textbf{0.24} & \textbf{0.79} & & \textbf{3.09} & \textbf{6.28} & \textbf{0.39} & \textbf{0.42} \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q3, batch size=40}} &  & \multicolumn{4}{c}{\textit{Q4, batch size=30}} \\  \cline{2-5} \cline{7-10} 
\textbf{Baseline} & 2.00 & 2.89 & 0.19 & 0.74 &  & 3.33 & 5.48 & 0.34 & 0.46 \\
\textbf{One-shot} &  \textbf{1.95} & \textbf{2.72} & \textbf{0.18} & \textbf{0.79} &  & \textbf{3.23} & \textbf{4.81} & \textbf{0.30} & \textbf{0.59} \\
\textbf{Self-reflection} &  2.55 &  3.21 & 0.21 & 0.74 &  & 3.85 & 5.55 &  0.35 &0.42 \\
\textbf{Batching} & 2.98 & 3.95 & 0.26 & 0.44 & & 3.83 & 5.93 & 0.37 & 0.32 \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q5, batch size=40}} &  & \multicolumn{4}{c}{\textit{Q6, batch size=20}} \\  \cline{2-5} \cline{7-10} 
 \textbf{Baseline} & 6.00 & 8.07 & 0.30 & 0.66 &  & 11.00 & 14.6 & 0.36 & \textbf{0.22} \\
\textbf{One-shot} &  \textbf{4.15} & \textbf{6.07} & \textbf{0.22} & \textbf{0.78} &  & \textbf{7.95} & \textbf{10.23} & \textbf{0.26} & \textbf{0.22} \\
\textbf{Self-reflection} & 7.33 & 9.46 & 0.35 & 0.57 &  & 10.90 & 14.53 & 0.36 & \textbf{0.22} \\
\textbf{Batching} & 8.20 & 10.33 & 0.38 & 0.63 & & 11.91 & 16.45 & 0.41 & 0.21 \\ \hline 
\end{tabular}%
}
\end{table}
%%



\subsection{Evaluations of Prompt Strategies in Grading}
\label{s:eval_prompts}


In this section, we assess the impact of different prompting strategies on performance during the grading process. The evaluation results are presented in Table~\ref{tab-prompts}. The \emph{batch size} in the table corresponds to the setting of the Batching prompts.
For all questions in the \ourdataset~dataset, our prompting strategies exceeded the baseline levels. 
The results indicate that different questions have different optimal prompting strategies, with Batching and One-Shot performing the best among all strategies. We also observed that, in certain cases, some strategies could reduce the grading performance. These observations suggest that it is crucial to design different prompting strategies tailored to the characteristics of specific questions.



% The results in Table~\ref{tab-selfreflection} shows the performance of the self-reflection prompt on the OS dataset. Notably, we observe variations in grading accuracy across different questions. Specifically, for questions \textit{Q1}, \textit{Q2} and \textit{Q6}, the self-reflection prompt achieves better grading accuracy compared to the baseline's initial performance.
% However, for questions \textit{Q3}, \textit{Q4} and \textit{Q5}, the grading results following self-reflection are worse than the baseline's initial performance. This variability underscores the question-dependent nature of LLMs' self-reflection ability in grading tasks.
% These findings highlight the importance of analyzing each question individually in the grading process. It emphasizes the inadequacy of employing a universal prompt strategy to achieve consistently high grading results across all question types. Instead, a flexible approach is warranted, wherein different strategies are adopted based on the specific characteristics of each problem.

% Moreover, these results validate the necessity of our proposed systematic and multi-agent grading framework, which allows for adaptable and context-specific grading strategies tailored to the nuances of each question.


% \xwj{Batching Table , add a note to explain the batch size value setting, like : Due to the token length limitation and varying lengths of questions and student answers for each question, the maximum batch size for grading differs for each question within the allowable token length range.}

% Table \ref{tab-batchos} and Table \ref{tab-batchmohler} show the grading results of the batching strategy on the OS dataset and the Mohler dataset, respectively. On the OS dataset, we find that the impact of the batching strategy on the grading performance across different questions is similar to the impact of the self-reflection strategy (as shown in Table \ref{tab-selfreflection}). Specifically, for $q_1$, $q_2$, $q_4$, and $q_5$, the grading accuracy with batching is better than without batching. However, for $q_3$ and $q_6$, the grading results with batching are better.
% On the Mohler dataset, we observe that the performance of the without batching prompt is better than the with batching approach.
% These findings further reinforce the point we claim based on the results in Table \ref{tab-selfreflection}, indicating that the effectiveness of some prompt strategies, such as self-reflection and batching, is highly dependent on the specific characteristics of the assessment tasks.
% The grading results from Table~\ref{tab-batchos} for the OS dataset and Table~\ref{tab-batchmohler} for the Mohler dataset shed light on our batching strategy's impact. 
% We find that effects of the batching strategy on the OS dataset closely resemble those observed with the self-reflection strategy as detailed in Table~\ref{tab-selfreflection}. Specifically, for questions \textit{Q1}, \textit{Q2}, \textit{Q4}, and \textit{Q5}, grading accuracy improves with batching compared to without batching. Conversely, for \textit{Q3} and \textit{Q6}, grading results without batching are better. 
% On the Mohler dataset, grading results without batching outperform those with batching, corroborating our point from Table~\ref{tab-selfreflection}. This highlights that the efficacy of prompt strategies like self-reflection and batching depends on assessment task characteristics.



\subsection{Evaluations for Score Review}


In this section, we evaluate the impact of the review process on grading performance and the effectiveness of re-grouping strategies in improving the accuracy of identifying unreasonable results.

\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \caption{Evaluation of re-grouping strategy}
    \label{tab-regroup}
    \resizebox{.55\textwidth}{!}{%
        \begin{tabular}{rcccccc}
        \hline
         & \multicolumn{6}{c}{\textbf{Accuracy $\uparrow$}} \\ \cline{2-7} 
        \textbf{Methods} & \textit{Q1} & \textit{Q2} & \textit{Q3} & \textit{Q4} & \textit{Q5} & \textit{Q6} \\ \hline
        \textbf{Baseline} & 0.58 & 0.64 & 0.59 & 0.72 & 0.55 & 0.70 \\
        \textbf{Re-grouping} & \textbf{0.62} & \textbf{0.73} & \textbf{0.71} & \textbf{0.77} & \textbf{0.64} & \textbf{0.76} \\ \hline
        \end{tabular}
    }
\end{wraptable}

% In this section, we evaluate the impact of the review process on grading performance and the effectiveness of re-grouping strategies in improving the accuracy of identifying unreasonable results. 
%
During the testing process, we randomly selected some students and modified their scores to simulate the occurrence of unreasonable results. The evaluation results are presented in Table~\ref{tab-regroup}.
%
The results show that through the review process, the LLM can detect anomalies in the grading, thereby further improving the accuracy. Additionally, the re-grouping strategy can further enhance the model's accuracy.


% For the OS dataset, which was manually annotated, each question comprises a total of 40 student responses, with the average of three grades serving as the correct ground truth label for each response.
% To simulate instances of erroneous scoring, we randomly selected 5 student responses for each question and constructed anomalous scores for these samples. This process allowed us to create a dataset containing instances of scoring errors.
% Subsequently, we employed the method proposed in Section~\ref{s:score_review} to leverage the GPT-3.5 model in identifying cases of anomalous scoring. By doing so, we aimed to evaluate the model's capacity to detect instances where the assigned score deviated from the correct ground truth label. This evaluation is crucial within the context of score review and quality assurance, as it enables us to assess the model's effectiveness in identifying scoring discrepancies.


\iffalse
这部分实验数据支撑比较少，我倾向于弱化实验效果， 强调提供一种新的思路：对input data的组织方式也会影响LLMs的任务效果。
\fi
% The experiment implementation details of this part can be found in the Appendix \ref{appedix:score_review}. Table \ref{tab-regroup} shows the performance of the regroup strategy on the score review task. Compared to the baseline method, our proposed regroup strategy achieved better accuracy performance in identifying anomalous scoring cases.
% Our main goal is to provide a new idea to constructing prompt strategies: The way we organize the input data can also influence the performance of LLMs on specific tasks, such as the score review task.
% In the future, we will continue to conduct related work to further explore this issue in depth. 








==> intro.tex <==
\section{Introduction}
\label{s:intro}


Large Language Models (LLMs)~\citep{llm-glm,llm-gpt3,llm-llama2,llm-mistral,llm-opt} have significantly revolutionized the world academically and in industry by excelling in multiple Natural Language Processing (NLP) tasks~\citep{hugginggpt,metagpt,toolllm,gorilla}. 
These models possess a profound understanding of a vast array of knowledge, can perform efficient logical reasoning, and exhibit deep comprehension of natural language. 
Therefore, they have been extensively integrated into workflows across numerous sectors worldwide.


A promising application in higher education involves leveraging LLMs to enhance the \textit{grading} process for students~\citep{fagbohun2024beyond, divya2023automation, chang2024automatic}. 
The grading process involves assessing their work and performance, providing critical feedback, and finally assigning scores. 
As a key measure of evaluating students' learning progress, scores must be given accurately, consistently, and fairly.
Traditionally, grading requires educators to design a comprehensive rubric and meticulously review each student's answers, a process that is both time-consuming and labor-intensive~\citep{jauhiainen2024evaluating}. As a result, there is growing interest in using LLMs to assist in this process.


Using LLMs to assist the grading process can be categorized under the research domain of Automated Short Answer Grading (ASAG) systems~\citep{fagbohun2024beyond, divya2023automation,chang2024automatic,yoon2023short}.
Current state-of-the-art systems typically grade each answer according to predefined grading rubrics set as system instructions and provide potential feedback. However, they still face significant challenges in achieving optimal grading performance in the following aspects:
%%
\begin{itemize}
    \item \textit{Rubric Generation}~\citep{wang2024enhancing}: 
    Existing systems require educators to meticulously craft detailed grading rubrics for each question in advance. 
    This process requires a significant investment of effort and time, and it is further complicated by the fact that even minor variations in grading rubrics can result in markedly different grading results~\citep{doostmohammadi2024reliable}; and educators cannot predict which rubric will be the most effective.
    Additionally, the design of rubrics and the grading process are currently conducted independently. This separation means that rubrics cannot be tailored to consider students' actual answers during the design phase. For instance, in the case of open-ended questions, students' responses may not fall within the scope of the rubric's guidelines, making the grading results unreliable.
    %%
    \item \textit{Consistency \& Fairness}~\cite{achintalwar2024detectors,raina2024llm,liu2024aligning}: 
    An answer should receive the same score across multiple independent grading sessions; and similar answers should receive similar scores. 
    However, due to the inherent randomness and hallucinations~\cite{huang2023survey} of LLMs, the model might produce entirely different scores for the similar input. 
    Besides, existing ASAG systems grade each answer independently, lacking the means to evaluate the overall fairness of the grading process and to further optimize it.
\end{itemize}
%%
The complexity and open-ended nature of the questions being graded exacerbate these issues~\citep{cohn2024chain,jauhiainen2024evaluating}. For instance, some open-ended questions do not have a standard answer that can be well-defined with a single statement; complex questions may require multiple sub-steps for grading; and lengthy questions and answers might exceed the LLM's context length.
These challenges motivate us to propose a better approach to grading.


Human excellence in grading stems from their ability to perform \textit{systematic} assessments, which involve phased planning, adjustments, and reflection throughout the grading process. 
%
Specifically: 
1) Humans can not only create standard rubrics based on the questions but also refine these rubrics by considering students' responses, thereby enhancing their comprehensiveness.
2) During grading, humans can accurately apply these rubrics to provide accurate scores. They can also remember previous student scores, which aids in maintaining fairness and consistency.
3) After completing grading, humans can review the results, identify any unreasonable outcomes through comparison and reflection, and make necessary adjustments.

% Inspired by human grading methodologies, \textit{we propose a multi-agent grading system named ``\textbf{\oursystem}.''} 
% The grading process is divided into three distinct stages: \textit{rubric generation}, \textit{grading}, and \textit{post-grading review}.
% Figure \ref{fig:sys_framework} shows the framework of the system.
% %

\iffalse

Inspired by human grading methodologies, \textit{we propose a multi-agent grading system named \textbf{\oursystem}.}, which 以一种系统性的方式重新思考grading task。
具体来说，
The grading process is divided into three distinct stages: \textit{rubric generation}, \textit{grading}, and \textit{post-grading review}.
在rubric generation阶段，我们将学生的answers也纳入到rubric的生成的指导内容中，通过提出a sampling-based iterative generation method来对rubrics进行生成优化，使得rubric的设计变得更加具有针对性。
优化后的rubrics在第二阶段被用来指导LLM对学生的answers进行打分。在这个过程中，我们进一步考虑多种prompt strategies对grading效果的影响。
最后，所有学生的grading results将在post-grading review阶段被进行评估。通过分组比较的方式，LLM将找出那些unreasonable的results。他们可以被送到上一阶段进行重新grading。
Figure \ref{fig:sys_framework} shows the framework of the system.
\fi

% During the rubric generation stage, we introduce a sampling-based iterative generation method. 

% This approach involves sampling student responses and iteratively refining the rubric based them, ultimately arriving at an optimal grading standard. 
% To enhance the grading process, we explore various prompting strategies, including one-shot prompts, self-reflection prompts, and batching prompts.
% The review stage employs a group comparison technique to identify and address any unreasonable assessments.
% Our implementation utilizes several well-designed agents to perform the tasks associated with each stage. These agents are integrated into a workflow to complete the overall grading process efficiently.

Inspired by human grading methodologies, \textit{we propose a multi-agent grading system named \textbf{\oursystem} to rethink the grading task in a systematic manner}. 
Specifically, the grading process is divided into three stages: \textit{rubric generation}, \textit{grading}, and \textit{post-grading review}.
In the rubric generation stage, we incorporate students' answers into the rubric design. By introducing a sampling-based iterative generation method, we optimize the generation process to make rubrics more targeted and effective. 
The optimized rubrics are then used in the grading stage to guide LLMs in grading students' answers. During this process, we further explore the impact of various prompt strategies on performance.
Finally, in the post-grading review stage, all students' grading results are reviewed. Through a group comparison approach, the LLM identifies unreasonable results, which can then be sent back for re-grading. Figure \ref{fig:sys_framework} illustrates the framework of the system.

Furthermore, \textit{we have collected and open-sourced a dataset named \textbf{\ourdataset} for evaluating the performance of LLMs in grading tasks}. 
This dataset is derived from our undergraduate Operating Systems course and includes all questions from the tutorials and assignments, along with the students' answers. Each answer is also labeled with human-given scores.
%
We utilized this dataset, along with an open-source dataset Mohler~\cite{mohler2011learning}, to thoroughly evaluate our system. The experimental results demonstrated our system's excellent capability in grading tasks.


Our contributions are summarized as follows: 
We point out that current ASAG systems lack a systematic perspective in viewing the grading task; and therefore face challenges in rubric generation, grading consistency, and fairness for complex questions.
To address these issues, we are the first to propose systematically designing the assessment process to explore the potential of LLMs; and further introduce a multi-agent grading framework named \oursystem, which has the ability to plan, reflect, and adjust in multiple stages in grading tasks. To effectively evaluate the system's performance, we collected and open-sourced the \ourdataset~dataset. Comprehensive experiments conducted on this dataset and the Mohlar dataset demonstrate that our system can significantly improve the accuracy and reliability of grading tasks.







% \begin{center}\njx{--------- NIU Juxin ---------}\end{center}






% ------------------------------------------------------------------
















% \iffalse
% \begin{itemize}
%     \item grading是重要的，需要耗费人力时间
%     \item existing LLM的做法只使用single agent的方式，在pre-establied rubric指导下打分，(figure 1) 缺陷：
%         （1）忽略了assessment是涉及到多个复杂任务的系统性任务，现有的single agent能力有限，并且只关注了grade with pre-establish环节。
%         （2）忽略了grading rubric本身的质量问题对grading result的影响。
%     现在的llm grading导致对一些问题的grading accuracy performance效果不好。并且LLM-based ASAG systems are not yet achieving human-level expert evaluators for complex assessment tasks.
%     \item 描述human grading的过程，我们识别出人之所以打分效果好的原因，是因为把assessemnt task当作一种多任务的系统性工作，xxxx 
%     \item Inspired by human grading approah, 我们识别出要想打分打的好，应该具备三种能力：*****；
%     然后我们提出了******
%     \item Summarize our contribution: xxxxx
%     (1) grade like human, multi-agent-based framework, systemmatically *****
%     (2) 针对每个agent, 我们都提出了有效的prompt策略 ***** 
%     (3) 贡献了数据集
%     Note: 强调首次提出system对待assessment task, 首次探究quality of grading rubric对grading result的影响。
%     我们期望我们的工作能一种新的系统视角看待assessment task, 充分发挥llm在grading task中的潜能*******
     
% \end{itemize}
% \fi








% \begin{center}\njx{--------- EOS ---------}\end{center}

\iffalse %          XIE WENJING

Grading is fundamental to any educational process as an evaluation system reflecting invidual performance and a way to compare results across populations. Effective assessment needs to ensure correctness, consistency, and fairness. However, even expert evaluators require significant human effort to achieve these goals.

With the rapid development of Large Language Models (LLMs), automated short answer grading (ASAG) systems based on LLMs have emerged to alleviate the burden on humans\cite{?}. 
However, existing ASAG systems follow a single-agent approach, where only use a single model to grade answers guided by instructor-defined grading rubric\ref{matelsky2023large}. 
They ignore that the fact that the assessment task is actually a complex, systematic process involving multiple task flows. On the one hand, the existing approach neglects the influence of other factors on grading quality, such as the crucial impact of grading rubric quality on the grading results\cite{?}. On the other hand, the single-agent approach limits the capabilities of LLMs in addressing different sub-tasks that arise during the assessment. 

In human assessment processes, relying on a pre-created grading rubric and a single perspective can introduce bias and result in unstable outcomes. Recognizing this, best practices involve multiple stages, including the desigining of grading rubrics, grading answers, and score reviews. Each stage must be executed with high quality to produce final reasonable, accurate, and fair assessment results.
However, existing works lack systematic research and exploration of the assessment task. 
 And the LLM-based ASAG systems are not yet achieving human-level expert evaluators for complex assessment tasks \cite{ChallengeLLMJudge, chen2024humans, achintalwar2024detectors, liu2024aligning, yoon2023short}. 
 % In our practice experiment, LLMs often struggle with evaluating intricate questions or student responses, leading to poor evaluation performance.


Inspired by the human grading approach, \emph{we propose an ideal assessment system based on multi-agents to grade systematically in a human-judge manner with three key abilities: generating grading rubric, grading with rubric, identifying and calibrating any unreasonable assessment. }Our system enables each agent to employ various prompt strategies to achieve good performance in their respective sub-tasks, while the multi-agents communicate and collaborate to achieve high-quality final assessment results.

To summarize, the main contribution of our work is as follows:
\begin{itemize}
    \item 1. We propose a multi-agent-based framework that grades answers just like expert human graders, with ability of automatically generating grading rubric, grading scores with customized feedback, and review scores, all with the aim of achieving better assessment performance, as depicted in Figure \ref{fig:sys_framework}. To the best of our knowledge, this is the first systematic exploration of the potential of LLMs in grading tasks.
    \item 2. We propose various prompt strategies to ensure that each agent can effectively accomplish their respective tasks and collaborate to generate high-quality assessment results.
    \item 3. We provide a dataset based on a real-world Operating System course, OS dataset, that is specifically designed for the automated answer grading task. This dataset is intended to encourage further research in this crucial area of educational NLP.
\end{itemize}

% % 图1，靠左侧对齐，右侧文字环绕
% \begin{wrapfigure}[7]{l}{0.6\textwidth} % 图像靠左对齐，占页面宽度的一半
%   \centering
%   \includegraphics[width=0.55\textwidth]{Styles/figures/framework_traditional.png} % 图1的路径和宽度
%   \caption{Traditional assessment system framework}
%   \label{fig:sys_traditional}
% \end{wrapfigure}

\fi

==> method.tex <==



\begin{figure}[]
  \centering
  \includegraphics[width=1.\textwidth]{Styles/figures/framework-crop.pdf} 
  \caption{Overview of the {\oursystem}~system}
  \label{fig:sys_framework}
\end{figure}



\section{\oursystem}


\oursystem~is a multi-agent system designed to enhance the performance of LLMs in grading tasks. 
The system framework is illustrated in Figure~\ref{fig:sys_framework}.
The system consists of three stages: \textit{Rubric Generation}, \textit{Grading}, and \textit{Post-Grading Review}.
In the Rubric Generation stage, we refine the pre-established scoring criteria to enhance their accuracy and comprehensiveness. The optimized scoring criteria will be used for grading in the Grading stage. After grading is complete, in the Post-Grading Review stage, we examine all the grading results to ensure there are no unreasonable outcomes.
The subsequent sections will provide detailed explanations of each stage.



% \paragraph{Rubric Generation}
% %
% The Rubric Generation stage takes place before the grading tasks begin. 
% For each question to be graded, a pre-defined rubric created by humans is provided in advance; and we employ a self-reflection paradigm~\cite{madaan2024self} to iteratively enhance its accuracy and comprehensiveness.
% In each iteration, a random sample of responses is selected and provided to the LLM. The LLM utilizes these responses to refine the rubric from the previous iteration. This optimized rubric is then carried forward to the next iteration. After the final iteration, the refined rubric is adopted as the final version and progresses to the subsequent stage.
% Besides, we design different sampling strategies to further improve the quality of the rubric.


% \paragraph{Grading}
% %
% The grading stage adheres to the existing ASAG paradigm~\cite{divya2023automation}, wherein each student's response is evaluated individually. 
% For the evaluation process, the student's response, the question description, the improved rubric from the previous stage, and any additional necessary context and instructions are compiled into a prompt. This prompt is then inputted into the LLM for grading.
% We also develop three prompt strategies to further enhance performance.


% \paragraph{Post-Grading Review}
% %
% After all student responses have been scored, in this stage, a comprehensive review of the grading results is conducted. 
% Specifically, grading results are grouped and each group's results are batch-processed by the LLM. The LLM compares these responses to detect anomalies. If any discrepancies are found, those results are sent back to the previous stage for re-grading.
% Additionally, we introduce a re-grouping strategy to improve the accuracy of the identification. This strategy involves repeatedly shuffling and re-grouping student responses, allowing each response to be compared with a diverse array of others across multiple iterations.


% \subsection{Data Processing Agent}
% The data processing agent primarily focuses on segmenting and extracting relevant content from the assignments submitted by students. The agent then stores the data in a structured format to enable efficient processing by the subsequent agents.
% In our actual implementation, the data processing agent utilizes the function call functionally provided by OpenAI to extract the necessary structured information from the student submissions.



\subsection{Rubric Generation} 
\label{s-gencri}

In this section, we present our method for Rubric Generation.
The Rubric Generation stage takes place before the grading tasks begin.
%
Our aim is to optimize the rubric specifically based on students' actual answers, making the subsequent grading process more accurate and reliable.

The rubric generation process is completed through multiple iterations following a self-reflective paradigm~\cite{madaan2024self}.
Specifically, for each question to be graded, we have a pre-defined rubric created by humans and all the students' answers.
In each iteration, we will select a small sample from the students' answers and have humans score these answers and provide reasons for the scores. These scores and reasons will then be provided as samples to the LLMs to learn how to grade and to help formulate the rubric with improved qualities. This optimized rubric is then carried forward to the next iteration as the input. After the final iteration, the refined rubric is adopted as the final version and progresses to the subsequent stage.
%
Formally speaking, consider a question $q$, a pre-established rubric $r_0$, and a set of student answers $A = \{a_1, a_2, \ldots, a_n\}$. 
We define a sampling method $S$ such that $S: A \to A_m$, where $A_m \subseteq A$ and $|A_m| = m$ with $m \ll n$. After human grading, we obtain a set of answer-score pairs $\{(a_i, g_i) \mid a_i \in A_m\}$. 
Based on this, an iteration can be formalized as a process represented by 
\begin{equation}\label{alg:rubric-gen}
    r_{i+1} = O\left(r_i, \{(a_i, g_i)\}, p\right)
\end{equation}
where $p$ is the system prompt sent to the LLMs. 
By performing this process $t$ times, we derive an optimization sequence $\{r_0 \to r_1 \to \ldots \to r_t\}$, with $r_t$ being the final refined rubric.
The process $O$ involves combing $r_i$, $\{(a_i, g_i)\}$, and $q$ to form a prompt for the LLM to generate a refined rubric. We give the details in Appendix~\ref{appedix:prompt_generate_rurbric}.

% The process $O$ involves combining $r_i$, $\{(a_i, g_i)\}$, and $p$ to form the prompt. We give the details in Appendix~\ref{appedix:prompt_generate_rurbric}.
% \iffalse
% 过程O涉及将$r_i$, $\{(a_i, g_i)\}$, and $q$结合形成prompt，让LLM来生成refined rubric的。
% \fi

\paragraph{Sampling Methods}
%
The sampling method $S$ directly affects the quality of the rubric.
\textit{Random sampling} is the simplest method. In each iteration, we randomly select from the remaining students' answers. However, the sample points obtained through this method do not accurately reflect the distribution of student performance under the given grading rubric. 
We aim for the sampling results to adhere to this distribution, as such a sample distribution can better guide LLMs in learning the impact of the rubric on different types of student answers. Based on this, we propose the \textit{Score-Distribution-Aware Sampling} method.
%
The Score-Distribution-Aware Sampling method consists of two steps. 
In the first step, the LLM performs an initial grading of all student answers based on the current grading rubric and obtains a score for each answer. This initial results allow us to obtain the distribution of student scores under the current grading rubric, which can guide our sampling process.
In the second step, we conduct scoring based on this sampling. The goal is to ensure that the distribution of the $m$ selected samples closely matches the score distribution obtained from the initial assessment.
We use a stratified sampling algorithm~\cite{liberty2016stratified} to achieve this goal.
%
Formally, grading all student answers in set $A$ using the current rubric $r_i$ yields scores $\{g_j \mid a_j \in A\}$.
To sample $m$ points from $n$ total answers, we first divide these scores into $k$ strata $\{B_1, B_2, \ldots, B_k\}$, with each stratum $B_l$ containing answers within a specific score range. 
For each stratum $B_l$, we compute the proportion $p_l = |B_l|/n$. 
Then, we determine the number of samples for each stratum as $m_l = \lceil p_l \times m \rceil$. 
Finally, we randomly sample $m_l$ answers from each $B_l$ to form the sample set $A_m$ as follows.
\begin{equation}
    A_m = \bigcup_{l=1}^k \text{RandomSample}(B_l, m_l)
\end{equation}
%
In Appendix~\ref{appedix:sampling}, we provide the pseudocode implementations of these two sampling methods respectively.


% Crafting high-quality grading rubrics is a crucial yet challenging aspect of the assessment process. Several key issues arise in practical grading scenarios: (1) The task of creating comprehensive and well-designed grading rubrics is inherently labor-intensive and time-consuming for instructors. (2) Pre-established grading rubrics may not capture the full breadth of possible correct answers, leading to the omission of certain valid responses and potential grading errors. (3) The pre-established rubrics may differ significantly from the actual form and content of students' responses, introducing discrepancies between the students' understanding of the question prompt and the instructor's interpretation. In such cases, the pre-established rubrics may not be suitable and require reconsideration based on the actual responses of students to achieve more reasonable and accurate grading results.
% To address these challenges, we propose a Rubric Generation Agent that leverages the capabilities of LLMs to generate and iteratively improve grading rubrics based on the actual student responses. The goal is to develop more reasonable and comprehensive rubrics, ultimately leading to enhanced grading quality and fairness.
% To the best of our knowledge, this paper is the first exploration of the impact of grading rubrics on LLM-based automatic grading quality and how LLMs can be utilized to enhance the quality of grading rubrics.

% Given a question \(q\) and a pre-established grading rubric \(R\), all student responses result in a set of candidates \(C=\{r_1, r_2, .., r_n\}\) for each question \(q\). 
% The core idea of our method is first to sample \(m\) (where \(m \ll n\)) examples from the student responses. For each sampled response \(r_i\), human teachers perform an assessment and assign a score \(s_i\), referred to as \((r_i, s_i)\) pairs. These samples are considered to be more correctly scored case. 
% Next, we utilize prompts to engage LLMs, such as ChatGPT, to compare and analyze the differences between the pre-established grading rubric \(R\) and the sampled student responses along with their assigned scores \((r_i, s_i)\). 

% In this way, one the one hand, we except LLM to be able to analyze the difference between pre-established rubrics and actual students' answers, and on the other hand, to be able to analyze from these samples what scoring standards are expected by the human teacher.


% Finally, LLMs then incorporate the insights gained from these samples to update the grading rubric accordingly. We propose two rubric generation algorithms that utilize different sampling methods: 

% \textbf{Random Sampling}. \xwj{If rename the alg-1:"Random Sampling Rubric Generation (RSRG)" ?}
% In Algorithm \ref{alg_random}, we randomly select $m$ samples from the entire set of student responses $C$. These samples are then graded by human expert teachers, serving as the ground truth labels. Next, we utilize the question $q$, initial rubric $R$, and the sampled subset $E^*$ as input to the LLM, constructing the prompt for rubric updating and generation.

% \textbf{Uniform Sampling based on Score Distribution}. \xwj{If rename the alg-2:}
% The idea behind Algorithm \ref{alg_distribute} is to ensure that the sampled cases represent different types of student responses and grading scores as comprehensively as possible.
% In Algorithm \ref{alg_distribute}, in line 1, we directly utilize the initial rubric $R$ as a guide for the LLM to provide preliminary grading for all student responses. This enables us to easily obtain a labeled dataset $D$, where for each student response $r_i$, $\hat{s_i}$ represents the LLM's scoring result.
% By using the same grading criteria for all students, the LLM implicitly categorizes student responses. Motivated by this, lines 2-10 involve aggregating student responses based on score ranges.
% Subsequently, lines 10-14 perform a proportional sampling of student responses and scores within each score range.
% Similar to Algorithm \ref{alg_random}, these samples are then graded by human expert teachers and will be used for rubric updating and generation.



% \begin{figure}[]
%     \centering

% \end{figure}


% Figure \ref{fig:prompt_genri} shows the prompt remplate for LLMs to genearated rubric, as defined function \emph{LLMGeneate()} in Algorithm \ref{alg_random} and Algorithm \ref{alg_distribute}. The prompt consists of the instruction, all input data (Blue color part in Figure \ref{fig:prompt_genri}), and the variable ${sample\_studata}$  is the student response-socre pairs sampled through Algorithm \ref{alg_random} or \ref{alg_distribute}. The generated rubric contains reference answer and detailed scoring rules.


% \begin{figure}[htbp] 
%     \centering
%     \includegraphics[scale=0.58]{Styles/figures/prompt_generateCri-crop.pdf}
%     \caption{The prompt template for LLMs to generate rubric. We replace the blue colored slot with real text before querying the LLMs.}
%     \label{fig:prompt_genri}
% \end{figure}



\subsection{Grading}
\label{s-prompt}

In this section, we give the design of the Grading stage.
The grading stage adheres to the existing ASAG paradigm~\cite{divya2023automation}. 
For the evaluation process, the student's answers, the question description, the improved rubric from the previous stage, and any additional necessary context and instructions are compiled into a prompt. This prompt is then inputted into the LLM for grading.


\paragraph{Prompt Strategy}
%
The effectiveness of grading is directly influenced by the quality of the prompts. Therefore, at this stage, we implement three different prompt strategies: \textit{one-shot prompts}, \textit{self-reflection prompts}, and \textit{batching prompts}.
In Section~\ref{s:eval_prompts}, we will explore the impact of these prompt strategies on grading performance through experiments.
We now introduce each of these prompt strategies respectively as follows. 
%
\begin{itemize}
    \item \textit{One-Shot Prompts:} LLMs have a good ability for in-context learning. Therefore, when generating prompts, we provide an additional example for the LLM to learn from. Figure~\ref{fig:oneshot} shows an example of such a prompt.
    \item \textit{Self-Reflection Prompts:} In this prompting strategy, each student's answer is initially graded by the LLM. This is followed by several iterations where the LLM is asked to reflect on its previous output and provide a more robust score and rationale. Figure~\ref{fig:reflection} illustrates this strategy's workflow and provides a sample instruction for self-reflection.
    \item \textit{Batching Prompts:} In this prompting strategy, several students' answers are processed in batches and graded together by the LLM. By considering multiple students' answers jointly, the LLM can better maintain fairness and consistency across them. Figure~\ref{fig:batching} shows an example of such a prompt.
\end{itemize}
%


% After generating high-quality and reasonable rubrics using the agent described in the section \ref{s-gencri}, grading agent explores different strategies to enhance prompt effectiveness for grading tasks. In our paper, the grading task involves three subtasks: (1) assigning scores to student responses. (2) providing explanatory feedback for the given scores. (3) enabling the LLM to evaluate its own confidence in the assessment results.

% strategy 1: one-shot prompt
% \textbf{One-shot Prompt}.
% In Figure \ref{fig:zeroshot}, we provide an example of a one-shot prompt. In this example, the prompt specifies that the grading score should be range from 0 to \emph{full\_points}. The prompt includes a one-shot example (Brown color part in the Figure \ref{fig:zeroshot}) that demonstrates the assessment process, and requires LLM to output the assessment result in a specific format, including grading score, explanation feedback for the score, and confidence for the evaluation.


% strategy 2: self-reflexion prompt
% \textbf{Self-reflection Prompt}.
% Our paper explore that if that LLMs self-correcting themselves without any sort of grounded feedback. As shown in Figure \ref{fig:reflexion}, given all input data, LLMs firstly generate an initial output. Then, without providing any human feedback, LLMs are only given self-reflection instructions to encourage them to check and analyze their initial output and provid improved results.
% In comparison to the the popular self-refined strategy \cite{madaan2024self}, which requires feedback in each iteration, providing human feedback for every student response during the evaluation process can be highly labor-intensive. Our approach aims to leverage the self-reflection capabilities of LLMs to enhance grading quality without relying on human feedback.



%strategy 3: batching prompt
% \textbf{Batching Prompt}. 
% In current LLM-based automatic answer grading systems, the standard approach is to grade individual student responses one by one using a single prompt for each question. This means using the "one prompt - one question - one student response" method. In this paper, we propose a batching approach where multiple student responses are graded together using a single prompt. Specifically, the approach is "one prompt - one question - $N$ student responses," where $N$ represents the batch size set for grading at each iteration.

% Compared to the traditional one-by-one grading method, batching offers advantages in terms of token efficiency when grading the same number of student responses. This is because common instructions and other basic components in the prompt can be shared and reused across the batch. Additionally, using batching allows LLMs to analyze and evaluate multiple student responses simultaneously, which raises question about the impact on grading results and quality. To the best of our knowledge, there is currently no existing research exploring this aspect.

% %
% \begin{figure}[]
%     \centering
%     % 左侧的minipage
%     \begin{minipage}[c]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Styles/figures/oneshot-crop.pdf} % 调整图像的宽度为文本宽度
%         \caption{Example of one-shot prompt.} % 图1的标题
%         \label{fig:oneshot}
%     \end{minipage}
%     \hfill
%     % 右侧的minipage
%     \begin{minipage}[c]{0.48\textwidth}
%         \centering
%         % 图2的minipage
%         \begin{minipage}[t]{\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{Styles/figures/reflection-crop.pdf}
%             \caption{Self-reflection prompting strategy.}
%             \label{fig:reflection}
%         \end{minipage}\\ [10pt] % 在图2和图3之间添加一些垂直空间
%         % 图3的minipage
%         \begin{minipage}[t]{\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{Styles/figures/batching-crop.pdf}
%             \caption{Example of batching prompt.}
%             \label{fig:batching}
%         \end{minipage}
%     \end{minipage}
% \end{figure}

\begin{figure}[]
    \centering
    \begin{minipage}[b]{0.327\textwidth}
        \includegraphics[width=\textwidth]{Styles/figures/oneshot-crop.pdf}
        \caption{One-shot prompt} % 图1的标题
        \label{fig:oneshot}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.327\textwidth}
        \includegraphics[width=\textwidth]{Styles/figures/reflection-crop.pdf}
        \caption{Self-reflection prompt}
        \label{fig:reflection}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.327\textwidth}
        \includegraphics[width=\textwidth]{Styles/figures/batching-crop.pdf}
        \caption{Batching prompt}
        \label{fig:batching}
    \end{minipage}
\end{figure}




\subsection{Post-grading Review}
\label{s:score_review}

LLMs may produce unreasonable grading results due to randomness or hallucination issues. Therefore, a post-grading review of all results is conducted after all student responses have been scored. In this section, we detail the review method.


We adopt a group comparison method to review the grading results and identify all unreasonable items. 
Considering the question being graded $q$, the grade rubric $r$, and the set of $n$ students' answers $A = \{a_1, \ldots, a_n\}$. After the previous stages, we obtain a set of answer-score pairs, forming the set $D = \{(a_i, g_i)\}$.
Given a group size $c$, we randomly divide the elements of $D$ into $n/c$ groups, with each group $D_i = \{(a_{i,1}, g_{i,1}), \ldots, (a_{i,c}, g_{i,c})\}$. Our goal is to use an LLM to identify all anomalies within each group $D_i$.
Specifically, the LLM will be asked to check:
1) For each $(a_i, g_i)$, whether $g_i$ deviates significantly from the requirements of the scoring rubric $r$;
2) Whether there are significant inconsistencies among the scores of these $c$ answers.
The LLM will return all detected anomalies. This process can be represented as:
\begin{equation}
    \text{outlier} = E(q, r, p, D_i)
\end{equation}
where $p$ contains the system prompt and other necessary context and instructions.
The value of the group size $c$ depends on ensuring that batching these $c$ pairs together does not exceed the context length of the LLM.

%
\begin{wrapfigure}{r}{0.5\textwidth}
%\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Styles/figures/regroup-crop.pdf}
    \caption{Our proposed re-grouping strategy.}
    \label{fig:regroup}
%\end{figure}
\end{wrapfigure}


\paragraph{Re-Grouping Strategy}
%
Intuitively, by comparing each grading result with a wider variety of other results, we can further improve the accuracy of the review. Therefore, we propose a re-grouping strategy, which is illustrated in Figure~\ref{fig:regroup}. 
During the re-grouping process, each group is further divided into $k$ sub-groups. From each sub-group, a set of sub-groups is sampled and recombined to form new groups. These newly formed sub-groups are then sent to the LLM for review. 
This re-grouping strategy enables a greater mixture of grading results, which helps in identifying outliers while maintaining the overall data distribution characteristics of $n$, despite the limitations of token length.



\iffalse

为了进一步增加review的准确性，
We introduce a second round of review, where each sub-group is further divided into $k$ sub-sub-groups. From each sub-group, one set of sub-sub-groups is sampled and recombined to form a new sub-group, which is then sent to the LLM for review. This re-grouping strategy allows for a greater mixture of sub-groups used to identify outliers, while still adhering to the overall data distribution characteristics of $n$, given the limited token length.
The re-grouping strategy illustrated in Figure~\ref{fig:regroup}.

\fi



% In the traditional assessment process, the results from teachers or automated grading systems are typically considered as the final scores. However, in real teaching scenarios, both human and automated grading systems can make mistakes during the grading process, leading to significant score deviations where students may receive scores that are either too high or too low. Manually double-checking the grading results would be a heavy burden.

% To address this issue, this paper proposes a score review agent based on LLMs. This agent automates the process of reviewing the grading results, identifying cases with grading errors, and making corrections. By implementing this agent, we aim to reduce the likelihood of students receiving undeserved scores and promote a fairer assessment of their performance. 

% Let's consider a total of $D=\{(r_1,s_1),(r_2,s_2)...,(r_n,s_n)\}$ with $n$ answer-score pairs that need to be reviewed. As LLMs have a token length constraint, it is not feasible to process a large batch of $n$ question answers in a single input. Thus, we propose a method where, for a given question $q$, we send a batch of $c$ student responses to the LLM at a time, where $c << n$, ensuring it remains within the maximum token length limit.
% Firstly, we utilize prompts to direct the LLM to analyze a batch of student grading results and identify any cases it deems as having unusual scores, defined as \emph{outlier}:
% \begin{equation}
%     outlier = f(q, R, D), D=\{(r_1,s_1),(r_2,s_2)...,(r_n,s_n)\}
% \end{equation}
% where $q$ represents the question, $R$ is the rubric, and $(r_i,s_i)$ corresponds to the answer and grading result of student $i$. During the review process, the LLM assesses two aspects: (1) whether each individual $(r_i,s_i)$ significantly deviates from $R$, and (2) whether the scoring standard used across the $c$ student answers are consistent. By considering these two analyses together, LLMs is able to detect the case with unusual scoring patterns.

% As shown in Figure \ref{fig:regroup}, the baseline method divides $n$ into $\lceil n/c \rceil$ sub-groups and sequentially feeds each sub-group into $f$ to obtain \emph{outlier} identification results for each group. However, this grouping strategy compromises the integrity of the $n$ data, as each round of review can only compare within localized sub-groups.
% To preserve the integrity of the $n$ data, this paper proposes a re-grouping strategy as illustrated in Figure \ref{fig:regroup}. The first round adopts the baseline grouping approach. We introduce a second round of review, where each sub-group is further divided into $k$ sub-sub-groups. From each sub-group, one set of sub-sub-groups is sampled and recombined to form a new sub-group, which is then sent to the LLM for review. This re-grouping strategy allows for a greater mixture of sub-groups used to identify outliers, while still adhering to the overall data distribution characteristics of $n$, given the limited token length.



\section{\ourdataset~Dataset}
\label{s:os_dataset}


\begin{figure}[] 
\centering
\small
\begin{tabularx}{\textwidth}{Xc}
    \hline
    \multicolumn{2}{p{13.5cm}}{\centering\textbf{Question Description}} \\ % \hline
    \multicolumn{2}{p{13.5cm}}{\textbf{(Full points: 15)} Now let’s look at \verb|vector-avoid-hold-and-wait.c|. What is the main problem with this approach? How does its performance compare to the other versions (i.e., \verb|vector-global-order| and \verb|vector-try-wait|), when running both with \verb|-p| and without it?} \\ \hline
    \multicolumn{2}{p{13.5cm}}{\centering\textbf{Standard Answer \& Grading Criteria}} \\ % \hline
    \multicolumn{2}{p{13.5cm}}{
        (1) The main problem with this approach is that it is too coarse ...
        % : the global lock (which protects the acquisition of all the other locks) will be under contention even when the vectors being manipulated by each thread is different.  
        \textbf{(\textit{5 points})}
        (2) The run times under heavy contention ...
        % (without the \verb|-p| flag) very close to those for vector-global-order. 
        \textbf{(\textit{5 points})}
        (3) For the high parallelism (with the \verb|-p| flag) case, ...
        % \verb|vector-avoid-hold-and-wait| performs as it does under high contention, but about twice as slow as \verb|vector-global-order| under high parallelism. 
        \textbf{(\textit{5 points})}
    } \\ \hline % \hline
    \multicolumn{1}{p{10cm}}{\centering\textbf{Student Answers}} & {\centering\textbf{Human-Given Grades}} \\  % \hline
    \multicolumn{1}{p{10cm}}{The main problem is that the global lock holds the lock even when sometimes it is not necessary to avoid deadlock, it plays too safe. The performance ...
    % without \verb|-p|: global order better than avoid hold and wait better than try wait. But with \verb|-p|: global order better than try wait better than avoid hold and wait.
} & \makecell[c]{13, 10, 10} \\ % \hline
    \multicolumn{1}{p{10cm}}{The main problem with this approach is that it is too coarse: the global lock (which protects the acquisition of all the other locks) will ...
    % be under contention even when the vectors being manipulated by each thread is different. The run times under heavy contention (without the \verb|-p| flag) very close to those for \verb|vector-global-order|. For the high parallelism (with the \verb|-p| flag) case, \verb|vector-avoid-hold-and-wait| performs as it does under high contention, but about twice as slow as \verb|vector-global-order| under high parallelism. Consequently, the comparison between vector-global-order and \verb|vector-try-wait| holds here as well.
    } & 15, 13, 15 \\ \hline
\end{tabularx}
% \includegraphics[width=1\textwidth]{Styles/figures/example_os.png}
\caption{An example from our OS dataset.
% with a question, the correct answer, and two student answers.
%The code involved in the question can be accessed and run by students on the server of the simulate environment. 
}
\label{fig:example_os}
\end{figure}



We have collected and open-sourced a dataset named \ourdataset, aimed at assisting researchers in evaluating the capabilities of LLMs in grading tasks. 
% 
The dataset is sourced from the Operating Systems course of undergraduate students at Computer Science department of City University of Hong Kong.
%\textit{Anonymous University}. 
The dataset includes 6 questions, selected from the course's tutorials and assignments. 
Figure \ref{fig:example_os} shows one question from the dataset, along with answers from two students.
% 
Each question contains a detailed description and necessary supplementary materials (such as executable code), along with the total score value, standard answers, and detailed grading criteria.
For each question, we collected answers from 40 students. These student answers were human-graded, with each answer being evaluated by three teaching assistants. 
The scores ranged from 0 to the maximum score for that question. 
Ultimately, the average of the three human scores was used as the student’s final score. 
% Figure \ref{fig:example_os} shows a question-answer pair from the dataset, along with example answers from two students.


% We create a data set of questions from Operating System assignments with answers provided by a class of undergraduate students. The assignments were administered as part of a Operating System course at the \textit{Anonymous University}. 
% For each assignment, the student answer sheets were collected via online system. The student submitted answers to 6 questions spread across 7 tutorials and 2 assignments. Figure \ref{fig:example_os} shows a question-answer pairs with two sample student answers each. 50 students were enrolled in the class and submitted answers to these assignments. The data set we work with consisted of a total of 240 student answers. 
% % This is less than the expected $50 \times 6 = 300$  as some students did not submit answers for a few assignments. 

% The answers were independently graded by three human graders, using a score from 0 (completely incorrect) to the \emph{full\_points} (perfect answer) for that question (\emph{full\_points} could vary across different questions), with a minimum granularity of 0.5 points. All human graders were PhD students in the computer science department and were teaching assistants for the Operating Systems course, and grader 3 was one of the authors of this paper. We treat the average grade of the three annotators as the gold standard against which we compare the output of our system.


==> related.tex <==
\section{Related Work}

% \xwj{finished rewritting}


% \njx{TO XIE.: If you want to cite references using a numeric format, use the command $\texttt{citep}$; and if cite references using the author+number format, use the $\texttt{citet}$ command. \textbf{ALWAYS ADD} a $\sim$ before the citation, and \textbf{DO NOT} manually type the authors.}

% \njx{\textbf{Example 1}: There is a surge in research interest in the field of large language models (LLMs) due to their exceptional performance across a wide range of tasks~\citep{brown2020language, thoppilan2022lamda, chowdhery2023palm, hoffmann2022training, OpenAI_report}...}
% \njx{\textbf{Example 2}: \citet{yoon2023short} use one-shot prompts to provide both analytic scores and final holistic scores for short answers consisting of multiple sub-questions.}


% \njx{To XIE.: DO NOT use $\textbackslash\texttt{vspace}$ to change the margin. This is forbidden!}

% \njx{To XIE.: For inserting a figure, typically DO NOT use $\texttt{htpb}$; leave it blank. \\ Use $\texttt{width=...}$ and $\textbackslash\texttt{textwidth}$ to specify a relative width based on page width. DO NOT use $\texttt{scale=...}$ to specify absolute width. \\ Leave several blank lines before and after the figure insertion statements.}



% There is a surge in research interest in the field of large language models (LLMs) due to their exceptional performance across a wide range of tasks ~\citep{brown2020language, thoppilan2022lamda, chowdhery2023palm, hoffmann2022training, OpenAI_report}. A crucial application is to utilize LLMs as evaluators for automatic answer grading ~\citep{fagbohun2024beyond, divya2023automation, chang2024automatic}.
% Existing works ~\citep{pinto2023large,song2024automated,henkel2023can} have demonstrated the capability of ChatGPT in understanding semantic details to grade open-ended question answers and provide feedback.
% ~\citet{nilsson2023gpt} use GPT-4 to grade programming assignments, proving the effective grading capabilities of LLMs for code-based responses.
% Extensive research efforts have also focused on leveraging advanced prompt engineering to enhance the grading results of LLMs.~\citet{yoon2023short} uses one-shot prompts to provide both analytic scores and final holistic scores for short answers consisting of multiple sub-questions.
% ~\citet{cohn2024chain} propose Chain-of-Thought prompts to enable LLMs to reason and evaluate the steps of student scientific experiments.
% Comparative prompt~\citep{liusie2024llm} and Rankprompt~\citep{hu2024rankprompt} transform direct score grading tasks into comparative assessment tasks, using relative comparison prompts to leverage LLMs for grading.~\citep{madaan2024self} propose Self-Refine prompts to improve initial outputs from LLMs through iterative feedback and refinement.~\citet{hasanbeig2023allure} introduce ALLURE, an iterative approach that compares LLM-generated evaluations with annotated data, and then incorporates human feedback for the next iteration. However, this iterative method requires annotated data and human feedback, which can be challenging to apply in real-world, large-scale answer grading scenarios.~\citet{del2023gradeaid} propose the GradeAid framework for real-time automatic short answer grading in educational contexts. Additionally, some studies~\citep{latif2024fine, song2024automated} have explored fine-tuning LLMs for specific types of short answer questions, but this approach requires collecting large-scale datasets and fine-tuning LLMs, which can be a non-trivial task.

% While LLMs have shown promising results in automatic grading tasks, there are still limitations in their real-world grading applications, and the quality of LLM grading has not yet reached the level of professional human graders~\citep{ChallengeLLMJudge, chen2024humans}.~\citet{liu2024aligning} study the misalignment between LLM evaluators and human judgment, revealing that existing calibration methods aimed at mitigating biases are insufficient for effectively aligning LLM evaluators.~\citep{doostmohammadi2024reliable} found that while automatic evaluation methods can approximate human judgments under specific conditions, their reliability is highly context-dependent. The papers~\citep{achintalwar2024detectors} and~\citep{raina2024llm} delve into the challenges of applying these models from the perspective of safety and reliability. 

% The existing methods take a single-agent approach to grading, without systematically decomposing the complex assessment tasks. Distinct from these approach, we advocate that LLMs should grade like humans, by exploring LLMs in assessment tasks from a systematic perspective and leveraging a multi-agent approach to coordinate multiple LLMs to enhance the grading effectiveness.

There has been a surge in research interest in the field of LLMs due to their exceptional performance across a wide range of tasks~\citep{brown2020language, thoppilan2022lamda, chowdhery2023palm, hoffmann2022training, OpenAI_report}. A crucial application is utilizing LLMs as graders for automatic answer grading~\citep{fagbohun2024beyond, divya2023automation, chang2024automatic}.
Existing works~\citep{pinto2023large, song2024automated, henkel2023can} have demonstrated the capability of ChatGPT in understanding semantic details to grade open-ended question answers and provide feedback. For instance, \citet{nilsson2023gpt} used GPT-4 to grade programming assignments, proving the effective grading capabilities of LLMs for code-based responses.
Extensive research efforts have also focused on leveraging advanced prompt engineering to enhance the grading results of LLMs. \citet{yoon2023short} employed one-shot prompts to provide both analytic scores and final holistic scores for short answers. \citet{cohn2024chain} proposed Chain-of-Thought prompts to enable LLMs to reason and evaluate the steps of student scientific experiments. Comparative prompt~\citep{liusie2024llm} and Rankprompt~\citep{hu2024rankprompt} transform direct score grading tasks into comparative assessment tasks, using relative comparison prompts to leverage LLMs for grading. 
\citet{madaan2024self} introduced Self-Refine prompts to improve initial outputs from LLMs through iterative feedback and refinement. \citet{hasanbeig2023allure} presented ALLURE, an iterative approach that compares LLM-generated evaluations with annotated data and then incorporates human feedback for the next iteration. However, these iterative methods require annotated data and human feedback, which can be challenging to apply in real-world, large-scale answer grading scenarios. \citet{del2023gradeaid} proposed the GradeAid framework for real-time automatic short answer grading in educational contexts.
Additionally, some studies~\citep{latif2024fine, song2024automated} have explored fine-tuning LLMs for specific types of short answer questions, but this approach requires collecting large-scale datasets and fine-tuning LLMs, which can be a non-trivial task.

While LLMs have shown promising results in automatic grading tasks, there are still limitations in their real-world grading applications, and the quality of LLMs grading has not yet reached the level of professional human graders~\citep{ChallengeLLMJudge, chen2024humans}. \citet{liu2024aligning} studied the misalignment between LLM evaluators and human judgment, revealing that existing biases. \citet{doostmohammadi2024reliable} found that while automatic evaluation methods can approximate human judgments under specific conditions, their reliability is highly context-dependent. The papers~\citep{achintalwar2024detectors} and~\citep{raina2024llm} delve into the challenges of applying these models from the perspective of safety and reliability.

Distinct from these approaches, our proposed \oursystem~system is the first to conduct a systematic study of the grading process, which we have divided into three stages: grading rubric generation, grading, and post-grading review. LLMs collaborate as multi-agents across these three stages, ultimately producing accurate, consistent, and fair grading results.



% Existing methods predominantly adopt a single-agent approach to grading, without systematically decomposing complex assessment tasks. Distinct from these approach, we advocate that LLMs should grade like humans by exploring LLMs in assessment tasks from a systematic perspective and leveraging a multi-agent approach to coordinate multiple LLMs to enhance grading effectiveness.

% \iffalse
% 与这些方法不同的是，我们提出的Grade-like-a-human system是第一个对打分过程进行系统性研究，并将其分成grading rubric的制作，打分，以及分数复查三个阶段。基于LLMs以multi-agent的方式在三个阶段之间相互协作，最后输出正确，一致且公平的打分结果。
% \fi




% %%%%%%%%%% cite in introduction
% (end of related work)
% multi-agent in other application
% \cite{chan2023chateval}
% \cite{hong2023metagpt}
% \cite{seff2023motionlm}
% \cite{yang2023spatio}

% dataset

% mohler dataset \cite{mohler2009text, mohler2011learning}
% \cite{sonkar2024automated}
% \cite{zhuang2024toolqa}




==> table.tex <==
\section{Experiments}
\label{s:exp}

In this section, we implement our system and test it using the \ourdataset~dataset mentioned in Section \ref{s:os_dataset}, as well as an open-source dataset, Mohler~\citep{mohler2011learning,mohler2009text}. 
The Mohler dataset is a question-answer grading database in the ASAG field, with questions pertaining to computer science. The organization of the Mohlar dataset is identical to the \ourdataset~dataset shown in Figure \ref{fig:example_os}, but it does not include grading criteria. A more detailed introduction can be found in Appendix~\ref{appendix:mohler}.
Our system is deployed on a server equipped with two A100 GPUs and 400GB of memory.
When implementing our system, we utilized OpenAI's API~\cite{openai-api} as our LLM source, and employed LangChain~\cite{langchain} to implement the agents and workflows. 
To objectively evaluate our system's performance in the grading task, we used multiple evaluation metrics, including MAE and RMSE, among others. These metrics are detailed in Appendix~\ref{Appendix:eval_metric}. 
\xwj{Add exlain for "bar error" like:"In this paper, all experimental results represent the average of multiple repeated experiments.
}


\subsection{Evaluations of Various Generated Rubrics}


We first evaluate the impact of different rubrics on the grading effectiveness of LLMs and simultaneously verify the effectiveness of the algorithm proposed in Section~\ref{s-gencri}.
Table~\ref{tab-gencri} presents the evaluation results on the \ourdataset~dataset, while Table~\ref{tab-gencri-mohler} shows the evaluation results on the Mohler dataset.


The evaluation on the \ourdataset~dataset includes four different grading rubrics. Among them, the \textbf{Coarse-gr., TA} and \textbf{Fine-gr., TA} rubrics are both manually generated rubrics that we followed when scoring student answers. 
The difference is the granularity: The former provides only the standard answer, while the latter additionally includes a grading criteria, as illustrated in Figure~\ref{fig:example_os}. \textbf{Gen., Rand.} and \textbf{Gen., Distr.} are respectively derived from the two rubric generation algorithms we demonstrated in Section~\ref{s-gencri}.
The rubrics for the Mohler dataset differ. Since the Mohler dataset does not provide grading criteria, it includes only two rubrics: \textbf{Coarse-gr.}, which directly comes from the standard answer for each question included in the dataset, and \textbf{Fine-gr.}, which is generated using the rubric generation algorithm.
In Appendix~\ref{appendix:rubric}, we present several examples to illustrate the different rubrics.


% \paragraph{Rubric Granularity v.s. Performance}
We compared the performance using different granularities of rubrics. In Tables~\ref{tab-gencri} and~\ref{tab-gencri-mohler}, we observed completely opposite phenomena: for the \ourdataset~dataset, fine-grained rubrics significantly improved scoring performance, whereas for the Mohler dataset, fine-grained rubrics actually reduced scoring performance.
%
We attribute it to the differing difficulties of the two datasets. 
For the OS dataset, each question is relatively long and complex, involving multiple steps and often including code execution. For such problems, LLMs lack sufficient capability to provide correct answers on their own, so detailed rubrics help LLMs score correctly.
In contrast, the questions in the Mohler dataset are relatively simple. For example, one question in the Mohler dataset is: \textit{``What is the role of a prototype program in problem solving?''}
For such questions, the world knowledge of LLMs is sufficient to provide good answers, as well as to evaluate students' responses. Therefore, not overly constraining the LLMs can better leverage their abilities~\cite{patil2023gorilla}.
% 
Additionally, in Table~\ref{tab-gencri}, we further observe that our rubric generation algorithm can further improve the grading performance on complex questions.
%
Based on this, we claim that our approach is effective for complex problems and further demonstrate the importance of our \ourdataset~dataset for better evaluating the performance of LLMs on grading tasks.
%
Therefore, in the subsequent evaluation, we mainly focus on the improvements our method brings to the \ourdataset~dataset.

% In Table~\ref{tab-gencri}, we compare the performance of \textbf{Fine-gr., TA} and \textbf{Coarse-gr., TA}. The results show that the scores achieved with the \textbf{Fine-gr., TA} are better, indicating that, on the OS dataset, providing more detailed grading criteria can help LLMs learn the human-expected grading rules more effectively.
% When comparing the rubrics generated using our proposed sampling methods (\textbf{Gen., Rand.} and \textbf{Gen., Distr.}) with those specified by TAs (\textbf{Coarse-gr., TA} and \textbf{Fine-gr., TA}) at different granularities, our method-produced rubrics demonstrate superior grading performance. This validates the effectiveness of our iterative rubric generation based on actual student responses in improving rubric quality. Additionally, the \textbf{Gen., Distr.} rubric achieves the best grading performance across all questions.

% Moreover, in the Mohler dataset, as shown in~\ref{tab-gencri-mohler}, the \textbf{Fine-gr.} rubric yields worse grading performance compared to the \textbf{Coarse-gr.} rubric. This result suggests that overly detailed grading rubrics can sometimes misguide the LLMs, especially when grading simple questions and short student responses, leading to more errors. This further supports the necessity of iteratively optimizing the rubric in our grading framework, based on the specific questions and actual student responses.


%  In this paper, we evaluate the impact of different grading rubrics on grading results using the OS dataset we collected, as shown in Table \ref{tab-gencri}.
%  Table \ref{tab-gencri-mohler} presents the grading results of different types of grading rubrics on the Mohler dataset.


% The first two type rubrics in the table represent rubrics formulated by the expert teachers (TA) of the OS course. The \emph{Coarse-grained} rubric provides a relatively broad grading scale, indicating the number of sub-questions and their corresponding scores.
% The \emph{Fine-grained} rubric adds specific grading criteria and rules for each sub-question, building upon the Coarse-grained rubric. The \emph{Random} and \emph{Distribution} type rubrics correspond to the two methods for generating rubrics by LLMs discussed in Section ~\ref{s-gencri}. (Examples of various types of rubric content can be found in the Appendix ~\ref{appendix:rubric})

% We can observe the following from table ~\ref{tab-gencri}:

% \begin{enumerate}
%     \item Compared to the Coarse-grained rubric, the Fine-grained rubric exhibits smaller scoring errors on LLMs and demonstrates a stronger correlation with human grading. This suggests that a more detailed grading rubric leads to better grading accuracy performance on LLMs.
%     \item Compared to the rubric formulated by the expert teachers, the grading rubrics generated using the proposed Random and Distribution methods significantly improve the quality of grading, with the Distribution method showing greater enhancement. This validates the effectiveness of the proposed strategy in combining LLMs with real student responses to generate grading rubrics.
% \end{enumerate}

%  We can observe that setting a more detailed grading rubric actually leads to a significant decrease in grading accuracy performance. This finding aligns with our earlier point, demonstrating that for particularly simple questions and short student responses, a detailed grading rubric can restrict the ability of LLMs during the grading process. 


%  Due to the relatively simple nature of the questions in the Mohler dataset, which mainly assess concepts in computer science, the student responses are typically shorter in length. As a result, it is not suitable to use overly complex grading rubrics. 
 
% When utilizing LLMs for grading tasks, different types of data may require different types of grading rubric. It is important to flexibly adjust the rubric based on the specific circumstances in order to choose the most suitable rubric.



\begin{table}[htbp]
\centering
\caption{Results obtained on OS dataset}
\label{tab-gencri}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
 & \multicolumn{4}{c}{\textit{Q1}} &  & \multicolumn{4}{c}{\textit{Q2}} \\ \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 6.97 & 8.98 & 0.47 & 0.46 &  & 5.90 & 7.57 & 0.47 & 0.10 \\
\textbf{Fine-gr., TA} &  4.51 & 5.62 & 0.30 & 0.74 &  & 5.90 & 7.75 & 0.48 & 0.15 \\
\textbf{Gen., Rand.} & 4.42 & 5.65 & 0.30 & 0.75 &  & 5.95 & 7.65 & 0.48 & 0.32 \\
\textbf{Gen., Distr.} & \textbf{4.05} & \textbf{5.21} & \textbf{0.27} & \textbf{0.76} &  & \textbf{5.70}  & \textbf{7.46}  & \textbf{0.47} & \textbf{0.37} \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q3}} &  & \multicolumn{4}{c}{\textit{Q4}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 2.85 & 3.41 & 0.23 & 0.62 &  & 5.45 & 7.32 & 0.46 & 0.36 \\
\textbf{Fine-gr., TA} & 2.40 & 3.38 & 0.23 & 0.71 &  & 4.78 & 6.25 & 0.39 & 0.45 \\
\textbf{Gen., Rand.} & 2.50 & 3.50 & 0.23 & 0.72 &  & 4.10 & 5.83 & 0.36 & 0.55 \\
\textbf{Gen., Distr.} & \textbf{2.35} & \textbf{3.17} & \textbf{0.21} & \textbf{0.75} &  & \textbf{3.38} & \textbf{4.89}  & \textbf{0.31} & \textbf{0.60} \\ % \hline  % \hline
 & \multicolumn{4}{c}{\textit{Q5}} &  & \multicolumn{4}{c}{\textit{Q6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr., TA} & 10.90 & 13.10 & 0.49 & 0.53 &  & 9.22 & 12.86 & 0.32 & 0.42 \\
\textbf{Fine-gr., TA} & 9.62 & 11.77 & 0.44 & 0.49 &  & 10.55 & 12.83 & 0.32 & 0.47 \\
\textbf{Gen., Rand.} & 6.05 & 8.41 & 0.31 & 0.64 &  & 9.62 & 12.62 & 0.32 & 0.40 \\
\textbf{Gen., Distr.} & \textbf{6.03} & \textbf{8.21} & \textbf{0.30}  & \textbf{0.66} &  & \textbf{8.72} & \textbf{11.42} & \textbf{0.29} & \textbf{0.50} \\ \hline
\end{tabular}%
}
\end{table}
%%
\begin{table}[htbp]
\centering
\caption{Results obtained on Mohler dataset}
\label{tab-gencri-mohler}
\resizebox{0.96\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline  \hline
 & \multicolumn{4}{c}{\textit{Q1.1}} &  & \multicolumn{4}{c}{\textit{Q2.6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.78} & \textbf{1.02} & \textbf{0.29} & \textbf{0.69} & & \textbf{0.90} & \textbf{1.11} & \textbf{0.37} & \textbf{0.34}   \\
\textbf{Fine-gr.} & 1.67  & 2.06 & 0.59 & 0.03 & & 1.83 &  2.00 & 0.67 & 0.37 \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q2.7}} &  & \multicolumn{4}{c}{\textit{Q3.6}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.59} & \textbf{0.74} & \textbf{0.15} & \textbf{0.15} &  & \textbf{0.43} & \textbf{0.87} & \textbf{0.35} & \textbf{0.60} \\
\textbf{Fine-gr.} & 0.90 & 1.11 & 0.22 & 0.55 &  & 0.61 & 1.21 & 0.45 & 0.53 \\%  \hline % \hline
 & \multicolumn{4}{c}{\textit{Q4.2}} &  & \multicolumn{4}{c}{\textit{Q11.7}} \\  \cline{2-5} \cline{7-10} 
\textbf{Coarse-gr.} & \textbf{0.57} & \textbf{0.80} & \textbf{0.27} & \textbf{0.68} &  & \textbf{0.68} & \textbf{0.80} & \textbf{0.28} & \textbf{0.74} \\
\textbf{Fine-gr.} & 0.50 & 0.89 & 0.30 & 0.64 &  & 0.72 & 0.97 & 0.31 & 0.68 \\ \hline
\end{tabular}%
}
\end{table}
%%
\begin{table}[]
\centering
\caption{Results of different prompts on OS dataset}
\label{tab-prompts}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rccccccccc}
\hline
\rule{0pt}{1.1em} % 设置行高
 \textbf{Methods} & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ &  & \textbf{MAE} $\downarrow$ & \textbf{NRMSE} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{Perason} $\uparrow$ \\ \hline   \hline
 & \multicolumn{4}{c}{\textit{Q1, batch size=10}} &  & \multicolumn{4}{c}{\textit{Q2, batch size=40}} \\ \cline{2-5} \cline{7-10} 
\textbf{Baseline} & 4.28 & 5.81 & 0.31 & 0.73 &  & 7.35 & 9.58 & 0.60 & 0.30 \\
\textbf{One-shot} &  3.74 & 5.33& 0.28 & 0.77 &  & 5.70 & 7.46 & 0.47 & 0.37 \\
\textbf{Self-reflection} & 3.83 & 4.98 & 0.26 & 0.76 &  & 5.95 & 7.68 & 0.48 & 0.36 \\
\textbf{Batching} & \textbf{3.59} & \textbf{4.64} & \textbf{0.24} & \textbf{0.79} & & \textbf{3.09} & \textbf{6.28} & \textbf{0.39} & \textbf{0.42} \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q3, batch size=40}} &  & \multicolumn{4}{c}{\textit{Q4, batch size=30}} \\  \cline{2-5} \cline{7-10} 
\textbf{Baseline} & 2.00 & 2.89 & 0.19 & 0.74 &  & 3.33 & 5.48 & 0.34 & 0.46 \\
\textbf{One-shot} &  \textbf{1.95} & \textbf{2.72} & \textbf{0.18} & \textbf{0.79} &  & \textbf{3.23} & \textbf{4.81} & \textbf{0.30} & \textbf{0.59} \\
\textbf{Self-reflection} &  2.55 &  3.21 & 0.21 & 0.74 &  & 3.85 & 5.55 &  0.35 &0.42 \\
\textbf{Batching} & 2.98 & 3.95 & 0.26 & 0.44 & & 3.83 & 5.93 & 0.37 & 0.32 \\ % \hline % \hline
 & \multicolumn{4}{c}{\textit{Q5, batch size=40}} &  & \multicolumn{4}{c}{\textit{Q6, batch size=20}} \\  \cline{2-5} \cline{7-10} 
 \textbf{Baseline} & 6.00 & 8.07 & 0.30 & 0.66 &  & 11.00 & 14.6 & 0.36 & \textbf{0.22} \\
\textbf{One-shot} &  \textbf{4.15} & \textbf{6.07} & \textbf{0.22} & \textbf{0.78} &  & \textbf{7.95} & \textbf{10.23} & \textbf{0.26} & \textbf{0.22} \\
\textbf{Self-reflection} & 7.33 & 9.46 & 0.35 & 0.57 &  & 10.90 & 14.53 & 0.36 & \textbf{0.22} \\
\textbf{Batching} & 8.20 & 10.33 & 0.38 & 0.63 & & 11.91 & 16.45 & 0.41 & 0.21 \\ \hline 
\end{tabular}%
}
\end{table}
%%



\subsection{Evaluations of Prompt Strategies in Grading}
\label{s:eval_prompts}


In this section, we assess the impact of different prompting strategies on performance during the grading process. The evaluation results are presented in Table~\ref{tab-prompts} (\emph{batch size} corresponds to the setting of the Batching prompts).
%
For all questions in the \ourdataset~dataset, our prompting strategies exceeded the baseline levels. 
The results indicate that different questions have different optimal prompting strategies, with Batching and One-Shot performing the best among all strategies. We also observed that, in certain cases, some strategies could reduce the grading performance. These observations suggest that it is crucial to design different prompting strategies tailored to the characteristics of specific questions.



% The results in Table~\ref{tab-selfreflection} shows the performance of the self-reflection prompt on the OS dataset. Notably, we observe variations in grading accuracy across different questions. Specifically, for questions \textit{Q1}, \textit{Q2} and \textit{Q6}, the self-reflection prompt achieves better grading accuracy compared to the baseline's initial performance.
% However, for questions \textit{Q3}, \textit{Q4} and \textit{Q5}, the grading results following self-reflection are worse than the baseline's initial performance. This variability underscores the question-dependent nature of LLMs' self-reflection ability in grading tasks.
% These findings highlight the importance of analyzing each question individually in the grading process. It emphasizes the inadequacy of employing a universal prompt strategy to achieve consistently high grading results across all question types. Instead, a flexible approach is warranted, wherein different strategies are adopted based on the specific characteristics of each problem.

% Moreover, these results validate the necessity of our proposed systematic and multi-agent grading framework, which allows for adaptable and context-specific grading strategies tailored to the nuances of each question.


% \xwj{Batching Table , add a note to explain the batch size value setting, like : Due to the token length limitation and varying lengths of questions and student answers for each question, the maximum batch size for grading differs for each question within the allowable token length range.}

% Table \ref{tab-batchos} and Table \ref{tab-batchmohler} show the grading results of the batching strategy on the OS dataset and the Mohler dataset, respectively. On the OS dataset, we find that the impact of the batching strategy on the grading performance across different questions is similar to the impact of the self-reflection strategy (as shown in Table \ref{tab-selfreflection}). Specifically, for $q_1$, $q_2$, $q_4$, and $q_5$, the grading accuracy with batching is better than without batching. However, for $q_3$ and $q_6$, the grading results with batching are better.
% On the Mohler dataset, we observe that the performance of the without batching prompt is better than the with batching approach.
% These findings further reinforce the point we claim based on the results in Table \ref{tab-selfreflection}, indicating that the effectiveness of some prompt strategies, such as self-reflection and batching, is highly dependent on the specific characteristics of the assessment tasks.
% The grading results from Table~\ref{tab-batchos} for the OS dataset and Table~\ref{tab-batchmohler} for the Mohler dataset shed light on our batching strategy's impact. 
% We find that effects of the batching strategy on the OS dataset closely resemble those observed with the self-reflection strategy as detailed in Table~\ref{tab-selfreflection}. Specifically, for questions \textit{Q1}, \textit{Q2}, \textit{Q4}, and \textit{Q5}, grading accuracy improves with batching compared to without batching. Conversely, for \textit{Q3} and \textit{Q6}, grading results without batching are better. 
% On the Mohler dataset, grading results without batching outperform those with batching, corroborating our point from Table~\ref{tab-selfreflection}. This highlights that the efficacy of prompt strategies like self-reflection and batching depends on assessment task characteristics.



\subsection{Evaluations for Score Review}



\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \caption{Evaluation of re-grouping strategy}
    \label{tab-regroup}
    \resizebox{.55\textwidth}{!}{%
        \begin{tabular}{rcccccc}
        \hline
         & \multicolumn{6}{c}{\textbf{Accuracy $\uparrow$}} \\ \cline{2-7} 
        \textbf{Methods} & \textit{Q1} & \textit{Q2} & \textit{Q3} & \textit{Q4} & \textit{Q5} & \textit{Q6} \\ \hline
        \textbf{Baseline} & 0.58 & 0.64 & 0.59 & 0.72 & 0.55 & 0.70 \\
        \textbf{Re-grouping} & \textbf{0.62} & \textbf{0.73} & \textbf{0.71} & \textbf{0.77} & \textbf{0.64} & \textbf{0.76} \\ \hline
        \end{tabular}
    }
\end{wraptable}

In this section, we evaluate the impact of the review process on grading performance and the effectiveness of re-grouping strategies in improving the accuracy of identifying unreasonable results. 
%
During the testing process, we randomly selected some students and modified their scores to simulate the occurrence of unreasonable results. The evaluation results are presented in Table~\ref{tab-regroup}.
%
The results show that through the review process, the LLM can detect anomalies in the grading, thereby further improving the accuracy. Additionally, the re-grouping strategy can further enhance the model's accuracy.


% For the OS dataset, which was manually annotated, each question comprises a total of 40 student responses, with the average of three grades serving as the correct ground truth label for each response.
% To simulate instances of erroneous scoring, we randomly selected 5 student responses for each question and constructed anomalous scores for these samples. This process allowed us to create a dataset containing instances of scoring errors.
% Subsequently, we employed the method proposed in Section~\ref{s:score_review} to leverage the GPT-3.5 model in identifying cases of anomalous scoring. By doing so, we aimed to evaluate the model's capacity to detect instances where the assigned score deviated from the correct ground truth label. This evaluation is crucial within the context of score review and quality assurance, as it enables us to assess the model's effectiveness in identifying scoring discrepancies.


\iffalse
这部分实验数据支撑比较少，我倾向于弱化实验效果， 强调提供一种新的思路：对input data的组织方式也会影响LLMs的任务效果。
\fi
% The experiment implementation details of this part can be found in the Appendix \ref{appedix:score_review}. Table \ref{tab-regroup} shows the performance of the regroup strategy on the score review task. Compared to the baseline method, our proposed regroup strategy achieved better accuracy performance in identifying anomalous scoring cases.
% Our main goal is to provide a new idea to constructing prompt strategies: The way we organize the input data can also influence the performance of LLMs on specific tasks, such as the score review task.
% In the future, we will continue to conduct related work to further explore this issue in depth. 









While large language models (LLMs) have been used for automated grading, they have not yet achieved the same level of performance as humans, especially when it comes to grading complex questions. 
Existing research on this topic focuses on a particular step in the grading procedure: grading using predefined rubrics. However, grading is a multifaceted procedure that encompasses other crucial steps, such as grading rubrics design and post-grading review. There has been a lack of systematic research exploring the potential of LLMs to enhance the entire grading~process.

In this paper, we propose an LLM-based grading system that addresses the entire grading procedure, including the following key components:
1) Developing grading rubrics that not only consider the questions but also the student answers, which can more accurately reflect students' performance.
2) Under the guidance of grading rubrics, providing accurate and consistent scores for each student, along with customized feedback.
3) Conducting post-grading review to better ensure accuracy and fairness.
Additionally, we collected a new dataset named \ourdataset~from a university operating system course and conducted extensive experiments on both our new dataset and the widely used Mohler dataset. Experiments demonstrate the effectiveness of our proposed approach, providing some new insights for developing automated grading systems based on LLMs.

